Transformer-Empowered Content-Aware Collaborative Filtering

Knowledge graph (KG) based Collaborative Filtering is an effective approach to personalizing recommendation systems for relatively static domains such as movies and books, by leveraging structured information from KG to enrich both item and user representations. Motivated by the use of Transformers for understanding rich text in content-based filtering recommender systems, we propose Content-aware KG-enhanced Meta-preference Networks as a way to enhance collaborative filtering recommendation based on both structured information from KG as well as unstructured content features based on Transformer-empowered content-based filtering. To achieve this, we employ a novel training scheme, Cross-System Contrastive Learning, to address the inconsistency of the two very different systems and propose a powerful collaborative filtering model and a variant of the well-known NRMS system within this modeling framework. We also contribute to public domain resources through the creation of a large-scale movie-knowledge-graph dataset and an extension of the already public Amazon-Book dataset through incorporation of text descriptions crawled from external sources. We present experimental results showing that enhancing collaborative filtering with Transformer-based features derived from content-based filtering outperforms strong baseline systems, improving the ability of knowledge-graph-based collaborative filtering systems to exploit item content information.

==> content/abstract.tex <==
Collaborative Filtering (CF) is one of the potent penalization methods that Collaborative Filtering (CF) is one of the potent penalization methods that power recommender systems for relatively static items such as movies and books,
while knowledge graph (KG) plays an increasing important role in recent work of CF models and demonstrated its effectiveness in alleviating tranditional CF problems such as cold start and data sparsity.
Transformers have showed excellent results in powering Content-based filtering (CBF) recommendation and can extract content-aware features from items' content information such as movie/book descriptions.
However, the transformers' power has not been leveraged by recent advance in KG-based CF models.
This paper aims to strengthen KG-based CF models' recommendation power with that of transformer-based CBF models.
% However, though transformers have showed excellent results in content-based recommendation, recent advance in content-aware KG-based CF models has not found an efficient way to incorporate transformer's power
% \linjun{need background to illustrate this, say transformer based models show excellent results in content based recommendation, etc: the transformer's power} 
% of content-based filtering (CBF) models to extract content-based features, .
To achieve this, we extended a famous book dataset, Amazon-Book, with book summary texts, and collected a brand-new large-scale movie dataset with an enormous knowledge graph.
We proposed and evaluated (1) a powerful KG-based CF model, KMPN, that models user preference through meta preferences; (2) a variant of a powerful CBF model, NRMS, that is grounded on a large pre-trained transformer; 
(3) a fusion framework (CKMPN) with Cross System Contrastive Learning to learn an enhanced content-aware CF model by the pre-trained features of CBF models.


% (3) a hybrid fusion framework, CKMPN, built on top of these two that outperformed baselines with Cross System Contrastive Learning for learning towards a content-aware CF model.power recommender systems for relatively static items such as movies and books,
while knowledge graph (KG) plays an increasing important role in recent work of CF models and demonstrated its effectiveness in alleviating tranditional CF problems such as cold start and data sparsity.
Transformers have showed excellent results in powering Content-based filtering (CBF) recommendation and can extract content-aware features from items' content information such as movie/book descriptions.
However, the transformers' power has not been leveraged by recent advance in KG-based CF models.
This paper aims to strengthen KG-based CF models' recommendation power with that of transformer-based CBF models.
% However, though transformers have showed excellent results in content-based recommendation, recent advance in content-aware KG-based CF models has not found an efficient way to incorporate transformer's power
% \linjun{need background to illustrate this, say transformer based models show excellent results in content based recommendation, etc: the transformer's power} 
% of content-based filtering (CBF) models to extract content-based features, .
To achieve this, we extended a famous book dataset, Amazon-Book, with book summary texts, and collected a brand-new large-scale movie dataset with an enormous knowledge graph.
We proposed and evaluated (1) a powerful KG-based CF model, KMPN, that models user preference through meta preferences; (2) a variant of a powerful CBF model, NRMS, that is grounded on a large pre-trained transformer; 
(3) a fusion framework (CKMPN) with Cross System Contrastive Learning to learn an enhanced content-aware CF model by the pre-trained features of CBF models.


% (3) a hybrid fusion framework, CKMPN, built on top of these two that outperformed baselines with Cross System Contrastive Learning for learning towards a content-aware CF model.

==> content/backup/conclusion.tex <==
\section{Conclusion}
In order to explore fusing CBF into CF models for movie/book recommendation, this paper presented two datasets: (1) Amazon-Book-Extended which inherited from a popular book recommendation dataset and was newly extended by summary texts of books; (2) a brand-new large-scale movie recommendation dataset, Microsoft-Movie-Dataset, which was recently collected from user browser history and provides an enormous knowledge graph together with summary texts for movies.
Both datasets will be shared with the research community in order to facilitate the domain research.

To utilize the power of large transformer models in context-aware collaborative filtering,
this paper firstly proposed and evaluated a powerful CF model, KMPN, which utilizes \textit{Gated Path Graph Convolution Networks}, \textit{Soft Distance Correlation Loss}, and \textit{Reciprocal Ratio Negative Sampling} to outperform existing baseline models.
Then, a novel approach, \textit{Corss-System Contrastive Learning} of embeddings was proposed to fuse content-aware features from a CBF model, NRMS-BERT, and achieved the best performance in record.
We finally presented benchmark results on both datasets for comparison with future research.

==> content/backup/datasets.tex <==
\section{Datasets}
In this section, we introduce two new datasets for recommendation: 
(1) a large-scale high-quality movie recommendation dataset that was newly collected from real user behaviors (Sec.~\ref{sec:movie_dataset});
(2) Amazon-Book-Extended dataset that derives from Amazon-Book dataset~\cite{wang2019kgat} but was newly augmented with textual book descriptions to allow the evaluation of content-based recommender systems (Sec.~\ref{sec:amazon_dataset}).

\subsection{Microsoft Movie Dataset}
\label{sec:movie_dataset}
\subsubsection{Dataset Construction}
This dataset was formed by real user browsing behaviors that were logged by Microsoft Edge Browser between 13/05/2021 and 20/06/2021 (39 days in total).
Sensitivity of data and privacy was firstly removed by decoupling users' real identity (e.g. IP, account identifier) from the data and assigning each user an insensitive unique virtual identifier.
To link users' browsing history with movies, we exploited an enormous knowledge graph, Microsoft Satori, that consists of a vast number of entities and a rich set of relationships among them.
Entities with type ``movie'' were extracted together with their one-hop neighbors and edges.
As a result, a movie-specific sub-graph of Satori was ready for use.

Among billions of user browser logs, knowledge-graph entity linking was performed to match the titles of web pages with the movie titles in our refined movie-specific knowledge graph.
Movie entities were extracted using our internal service that provides NER and entity linking.

The next move is to refine user-movie interactions in order to make the dataset cleaner and more compact:
(1) Consecutive but duplicated user interactions on the same movie were merged to one single record. Browsing time (DwellTime) was aggregated.
(2) Users with less than 10 interactions in 39 days were dropped.
(3) The top frequent 50,000 movies with the most user interactions were selected.
% with the lowest user interaction count at 17.
% (3) Movies are ranked by the total amount of user interactions in 39 days, and first 50,000 movies are selected with the lowest user interaction count at 17.

After careful pre-processing and filtering, 125,218 active users with the most interactions in all days were chosen.
% They interacted with 50,000 movies in total. 
Knowledge-graph entities related to these 50,000 movies were extracted and formed a knowledge graph with 25,0327 entities (including movie items).
Each user is represented by [$UserID$, $UserHistory$], where $UserID$ is a unique identifier that has been delinked from real user identity, and $UserHistory$ is an ID list of movie items that the user has interacted with.

For training and evaluating recommender systems, $UserHistory$ was split into train/valid/test:
First 80\% of users' historical interactions (ordered by click date-time) are in the train set, 80\% to 90\% serves as the valid set, and the remaining is reserved for testing.
While validating or testing, interactions in the train set serve as users' previous clicked items and systems are evaluated on their ratings for test set items.

In addition to the traditional data split strategy, a cold-start user set was designed to help model evaluate its performance on users outside the training dataset.
3\% of users were moved to a cold-start set and they are not accessible by models at training.
This portion of interactions was split into a cold-start history set with first 80\% interactions of each user, and a test set with the remaining 20\%.



A comparison with some popular existing recommendation datasets is provided in Table~\ref{tab:comparison_with_datasets}.
\textbf{MovieLens-20M}\footnote{\href{https://grouplens.org/datasets/movielens/}{https://grouplens.org/datasets/movielens/}} is a popular benchmark that has been widely used, while
\textbf{Flixster}\footnote{\href{https://sites.google.com/view/mohsenjamali/flixter-data-set}{https://sites.google.com/view/mohsenjamali/flixter-data-set}} is large but less popular in recent work.
\textbf{Amazon-Book}~\cite{wang2019kgat}, \textbf{Last-FM}~\cite{wang2019kgat}, \textbf{Book-Crossing}~\cite{ziegler2005improving}\footnote{\href{http://www2.informatik.uni-freiburg.de/~cziegler/BX/}{http://www2.informatik.uni-freiburg.de/~cziegler/BX/}} and \textbf{Alibaba-iFashion}~\cite{wang2021learning} are dedicated for KG-based CF model evaluation.



It can be concluded that our new movie dataset consists of large-scale users and movies, and incorporates an enormous movie-specific knowledge graph with millions of triplets and entities, which has not been provided by existing popular movie recommendation datasets.
In addition, our dataset provides not only titles and genres (as in MovieLens-20M), but also other content-based information, specifically, rich summary texts of movies that enable content-based recommendation with large language understanding models (such as BERT, GPT-3).
% In addition, the dataset comprises rich texts of movie descriptions, which enable content-based recommendation with large language understanding models (such as BERT, GPT-3).


\begin{table*}[!ht]
\caption{Comparison with existing popular datasets for recommender systems.}
\label{tab:comparison_with_datasets}
\small
\begin{tabular}{llllllllll}
\toprule
Type     & Dataset                 & \#Users & \#Items & \#Interactions & Has KG? & \#Entities & \#Relations & \#Triplets & Has Descriptions?           \\ 
\midrule
% Movie    & MovieLens-25M           & 16,2000 & 62,000  & 25,000,000     & No              & N/A        & N/A         &            & No                      \\ 
Movie    & MovieLens-20M           & 138,000 & 27,000  & 20,000,000     & No              & N/A        & N/A         &    N/A        & No                      \\
Moive   & Flixster  & 1,002,796   & 66,730    & 1,048,576   & No    & N/A &   N/A & N/A & No\\
Book     & Amazon-Book             & 70,679  & 24,915  & 847,733        & Yes             & 88,572     & 39          & 2,557,746  & No                      \\ 
Book    & Book-Crossing   & 276,271   & 271,379  & 1,048,575 & Yes & 25,787 & 18 & 60,787 & No\\
Music    & Last-FM                 & 23,566  & 48,123  & 3,034,796      & Yes             & 58,266     & 9           & 464,567    & No                      \\ 
Shopping & Alibaba-iFashion        & 114,737 & 30,040  & 1,781,093      & Yes             & 59,156     & 51          & 279,155    & No                      \\
\midrule
Book     & Amazon-Book-Extended    & 70,679  & 24,915  & 847,733        & Yes             & 88,572     & 39          & 2,557,746  &  Yes       \\ 
Movie    & Microsoft-Movie-Dataset & 125,218 & 50,000  &  4,095,146              & Yes             & 250,327    & 12          & 12,055,581 & Yes\\
\bottomrule
\end{tabular}
\vspace{-0.3cm}
\end{table*}

\subsubsection{Statistical Analysis}
\label{sec:movie_statistical_analysis}
\begin{figure}
\centering     %%% not \center
\subfigure[Length of user interactions ($\mu=32.70$,$\sigma=45.76$)]{\label{fig:hist_number_user_interactions}\includegraphics[width=0.48\linewidth]{content/figures/number_user_interactions.png}}
\hfill
\subfigure[Interactions with movies ($\mu=83.33$,$\sigma=582.50$)]{\label{fig:hist_movie_interaction_count}\includegraphics[width=0.48\linewidth]{content/figures/movie_interaction_count.png}}\\
% \subfigure[Histogram of the DwellTime of interactions]{\label{fig:hist_dwelltime}\includegraphics[width=0.48\linewidth]{content/figures/dwelltime_count.png}}
% \hfill
\subfigure[Length of texts of Movie-Dataset ($\mu=425.22$,$\sigma=329.93$)]{\label{fig:hist_movie_text_length}\includegraphics[width=0.48\linewidth]{content/figures/text_length_count_movie.png}}
\hfill
\subfigure[Length of texts of Amazon-Book-Extended ($\mu=151.75$,$\sigma=206.98$)]{\label{fig:hist_book_text_length}\includegraphics[width=0.48\linewidth]{content/figures/text_length_count_amazon.png}}
\caption{Key statistics of Microsoft-Movie-Dataset (Fig.~\ref{fig:hist_number_user_interactions}-\ref{fig:hist_movie_text_length}) and  Amazon-Book-Extended (Fig.~\ref{fig:hist_book_text_length}).}
\label{fig:dataset_analysis}
\end{figure}
Fig.~\ref{tab:comparison_with_datasets} presents the key statistics of the dataset.
This dataset contains 125,218 users, 50,000 movie items, interactions. The knowledge graph contains 250,327 entities with 12 relation types and 12,055,581 triplets.
The attributes of movies include content-based properties (title, description, movie length) and properties already tied to knowledge graph entities (production company, country, language, producer, director, genre, rating, editor, writer, honors, actor).
Fig.~\ref{fig:hist_number_user_interactions}-\ref{fig:hist_movie_text_length}  show the distribution of length of interactions per user, number of interactions per movie, and length of movie descriptions respectively.
The average length of movie descriptions is 425 words, which is long enough to capture the story line of movies and infer preference.
The average number of user interactions is 32.70, providing rich resources for modelling users' long-term interest.
The first 19 days' of data (with similar data distribution but less users and interactions) is separated as ``Standard'' for most research purposes, while the full 39 days' are released as ``Extended'' for industry use.

\subsection{Extended Amazon Book Dataset}
\label{sec:amazon_dataset}
The original Amazon-Book dataset was released by ~\cite{wang2019kgat}, and was used as point for comparisons of many advanced recommendation systems.
However, this dataset can not satisfy the research need as it provides only CF interaction data without content-based features for CBF evaluation.
To fill this gap, we extended the dataset with descriptions extracted from multiple data source, as the dataset was collected in 2014 and many items have expired on the Amazon website.
The procedure is summarized as below:

(1) We matched product descriptions in Amazon with entries in Amazon-Book using their unique item identifiers (asin). 24,555 items were successfully matched (98.56\%).

(2) We then matched each of the remaining item with a most relevant entry in Microsoft Satori such that rich descriptions were extracted. 325 items were matched at this step.

(3) The rest 28 items were matched manually to most relevant products in Amazon.

Finally, we extracted rich texts for Amazon-Book dataset with more than 99.99\% match rate, leading to an extended dataset Amazon-Book-Extended.
The distribution of description lengths is given in Fig.~\ref{fig:hist_book_text_length}, with a mean length of 151.75.


==> content/backup/experiments.tex <==
\section{Experiments}

\begin{table*}[!ht]
\caption{Comparison of baseline models and our proposed models on Amazon-Book-Extended dataset. Numbers \underline{underlined} are existing state-of-the-art performance, while best performance of the proposed models are marked in \textbf{bold}.
Relative improvements over models are shown in the last two rows.
}
\label{tab:compare_baselines}
\small
\centering
\begin{tabular}{llllllllll}
\toprule
                                  & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{ndcg}   & \multicolumn{3}{c}{Hit Ratio}  \\
~                                 & @20   & @60   & @100    & @20   & @60     & @100  & @20   & @60   & @100        \\
\midrule
BPRMF                                & 0.1352&	0.2433&	0.3088&	0.0696&	0.09568&	0.1089&	0.2376&	0.3984&	0.4816

          \\
CKE                               & 0.1347&	0.2413&	0.3070&	0.0691&	0.09482&	0.1081&	0.2373&	0.3963&	0.4800
            \\
KGAT                              & 0.1527&	0.2595&	0.3227&	0.0807&	0.10655&	0.1194&	0.2602&	0.4156&	0.4931
       \\
KGIN                              & \underline{0.1654}&	\underline{0.2691} &	\underline{0.3298} &	\underline{0.0893} &	\underline{0.1145} &	\underline{0.1267} &	\underline{0.2805} &	\underline{0.4289} &	\underline{0.5040}
       \\
\midrule
KMPN & \textbf{0.1719} & 0.2793 & 0.3405   & \textbf{0.0931} & 0.1189 & 0.1315 & \textbf{0.2910} & 0.4421 & 0.5166       \\
- SoftDistanceCorrelation  & 0.1704 & 0.2790 & 0.3396   & 0.0924 & 0.1185  & 0.1310 & 0.2881 & 0.4419 & 0.5152       \\
- ReciprocalRatioNegativeSampling                              & 0.1690 & 0.2774 & 0.3391   & 0.0913 & 0.1177  & 0.1302 & 0.2872 & 0.4414 & 0.5155       \\
% KMPN                              & 0.1690 & 0.2774 & 0.3391   & 0.0913 & 0.1177  & 0.1302 & 0.2872 & 0.4414 & 0.5155       \\
% +ReciprocalRatioNegativeSampling  & 0.1704 & 0.2790 & 0.3396   & 0.0924 & 0.1185  & 0.1310 & 0.2881 & 0.4419 & 0.5152       \\
% +SoftDistanceCorrelation          & \textbf{0.1719} & 0.2793 & 0.3405   & \textbf{0.0931} & 0.1189 & 0.1315 & \textbf{0.2910} & 0.4421 & 0.5166       \\
\midrule
NRMS-BERT &	0.1142 &	0.2083	& 0.2671 &	0.0592 &	0.0817 &	0.0935 &	0.2057 &	0.3487 &	0.4273 \\
\midrule
CKMPN ($\lambda_{CS}=0.2$) & 0.1699 & 0.2812 & \textbf{0.3461}   & 0.0922 & 0.1190 & 0.1319 & 0.2880 & 0.4460 & 0.5235       \\
CKMPN ($\lambda_{CS}=0.1$) & 0.1718 & \textbf{0.2821} & 0.3460   & 0.0928 & \textbf{0.1197} & \textbf{0.1326} & 0.2908 & \textbf{0.4474} & \textbf{0.5244}   \\
\midrule
Improv. (\%) CKMPN v.s. Baselines &	3.90&	4.82&	4.94&	4.31&	4.55&	4.59&	3.72&	4.33&	4.04
\\
Improv. (\%) CKMPN v.s. KMPN & 0.0	& 1.0 &	1.6	 & -0.3	 & 0.7 &	0.8 &	0.0	& 1.2 &	1.5\\
\bottomrule
\end{tabular}
\end{table*}
In this section, we present experimental results of the three proposed models: KMPN, NRMS-BERT, and CKMPN, with detailed discussions.
We firstly demonstrate model improvements over existing baseline models including state-of-the-art models on Amazon-Book-Extended, which has an extensive record of publications that enables direct and fair comparison.
Then we provide benchmark results on our brand-new Microsoft-Movie-Dataset to enable the development and comparison of future models.


\subsection{Evaluation Metrics}
Following common practice~\cite{he2017neural, wang2019kgat, wang2021learning}, we report several metrics (algorithms summarized in \cite{krichene2020sampled}) for evaluating model performance:

\textit{Recall@K}: within top-$K$ recommendations, how well the system is able to recall the test-set browsed items for each user.

\textit{ndcg@K} (Normalized Discounted Cumulative Gain): increases when relevant items appear more earlier in the recommended list. 

% \textit{Precision@K}: how relevant the recommended top-$K$ items are to the specific user.

\textit{HitRatio@K}: how probable the user click through one of the recommended top-$K$ items.

\subsection{Baselines}
We take the performance of several recently published recommender systems as points for comparison.
We carefully reproduced all these baseline systems from their official repository.\footnote{As a result, the metrics reported in this paper may differ from what were presented in the original papers.}

\textbf{BPRMF}~\cite{rendle2012bpr}: an advanced matrix factorization method that applies a generic optimization criterion BPR-Opt for personalized ranking that derives from Bayesian analysis.


\textbf{CKE}~\cite{zhang2016collaborative}: a CF model that aims to leverage heterogeneous information in a knowledge base for recommendation.

\textbf{KGAT}~\cite{wang2019kgat}: Knowledge Graph Attention Network (KGAT) which explicitly models the high-order connectivities in KG in an end-to-end fashion. The models' user/item embeddings were initialized from the pre-trained \textbf{BPRMF} weights.

\textbf{KGIN}~\cite{wang2021learning}: A state-of-the-art CF model that models users' latent intents as a combination of KG relations.



% \subsection{Training Details}
% All experiments were run on 8 NVIDIA A100 Tensor Core GPUs with batch size $8192\times 8$ for KMPN/CKMPN and $4\times8$ for NRMS-BERT.
% KMPN/CKMPN's optimizer was Adam \cite{DBLP:journals/corr/KingmaB14} with 2000 epochs of linearly decayed learning rate from $10^{-3}$ to $0$ for Amazon-Book-Extended and $5\times10^{-4}$ to $0$ for Microsoft-Movie-Dataset.
% NRMS-BERT was optimized with Adam at a constant learning rate of $10^{-4}$.
% Codes will be released with all training details upon publication.


\subsection{Model Performance on Amazon Dataset}






Performance of models is presented in Table~\ref{tab:compare_baselines}. 
Our proposed CF model, KMPN, with \textit{Reciprocal Ratio Negative Sampling} and \textit{Soft Distance Contrastive Learning}, achieved a significant improvement on all metrics over the performance of the existing state-of-the-art model KGIN, for example, Recall@20 was improved from 0.1654 to 0.1719, Recall@100 from 0.3298 to 0.3405, and ndcg@100 from 0.1267 to 0.1315.

% As shown, enhanced by knowledge graph, our proposed collaborative-filtering model KMPN achieved an improvement on all metrics over the performance of the existing state-of-the-art model KGIN, for example, Recall@100 was improved from 0.3298 to 0.3391 and Hit Ratio@100 from 0.5040 to 0.5155.

NRMS-BERT models user-item preferences through only summary texts of items, without external information from a knowledge base.
It still achieves 0.1142 in Recall@20 and 0.4273 Hit Ratio@100, not far from the KGIN baseline at 0.5040 Hit Ratio@100. 
It suggests that our extension to Amazon-Book dataset serves as a good additional content-based source for constructing recommendation systems.

Finally, our proposed \textit{Cross-System Contrastive Learning} approach significantly improves all @60/@100 metrics while keeping model's performance of @20.
For example, as shown, CKMPN achieved 0.1718 in Recall@20, the same as the best configuration of KMPN.
But CKMPN (0.3461 Recall@100) outperforms KMPN (0.3405 Recall@100) by 1.6\%.
This demonstrates that by gathering item and user embeddings of one system (KMPN) towards those of the other system (NRMS-BERT) through proxies (Cross-System Contrastive Learning) encourages KMPN to learn and fuse content-aware features from the learnt representations of a CBF model.
The fuse of this content-based feature significantly enhanced KMPN's ability to gather more relevant items into the top-$100$ recommendation list.
This improvement on top-$60/100$ metrics is appealing to the industry where a relatively large amount of items are firstly recalled by a Recall Model and then a Ranking Model is adopted to refine the list ranking.

In the following subsections, we briefly explore the effects brought by the hyperparameters in order to support the rationale of our designs for KMPN.
\begin{table*}[!ht]
\caption{Benchmark results on Microsoft-Movie-Dataset. Best performance is marked in \textbf{bold}.
}
\label{tab:compare_baselines_movies}
\centering
\small
\begin{tabular}{llllllllll}
\toprule
                                  & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{ndcg}   & \multicolumn{3}{c}{Hit Ratio}  \\
~                                 & @20   & @60   & @100    & @20   & @60     & @100  & @20   & @60   & @100        \\
\midrule
BPRMF                                & 0.1387 &	0.1944&	0.2206&	0.0961&	0.1137&	0.1192&	0.1980&	0.2785&	0.3236
          \\
CKE & 0.1369&	0.1898&	0.2150&	0.0940&	0.1108&	0.1160&	0.1950&	0.2707&	0.3155
\\
KGAT&	\underline{0.1403}&	0.1928&	0.2185&	\underline{0.1006}&	0.1173&	0.1226&	0.1997&	0.2742&	0.3196
\\
KGIN&	0.1351&	\underline{0.2119}&	\underline{0.2445}&	0.0982&	\underline{0.1254}&	\underline{0.1322}&	\underline{0.2194}&	\underline{0.3081}&	\underline{0.3643}\\

\midrule
KMPN & 0.1434&	0.2130&	0.2427&	0.1073&	0.1305&	0.1367&	0.2193&	0.3098&	0.3602
\\
NRMS-BERT& 0.0941&	0.1456&	0.1598&	0.0754&	0.0914&	0.0945&	0.1541 & 0.2034&	0.2348
\\
CKMPN & \textbf{0.1463}&	\textbf{0.2153}&	\textbf{0.2467}&	\textbf{0.1087}&	\textbf{0.1334}&	\textbf{0.1402}&	\textbf{0.2211}&	\textbf{0.3124}&	\textbf{0.3657}
\\



\bottomrule
\end{tabular}

\end{table*}




\subsubsection{Effects of Reciprocal Ratio Negative Sampling}
\label{sec:experiments:negative_sampling}
Through \textit{Reciprocal Ratio Negative Sampling}, KMPN further improves the metrics: Recall@20 increases from 0.1690 to 0.1704.
In line with our intuition, reducing the probability of sampling popular items as negative samples for training can significantly benefit the model learning.
This demonstrates that while viewed-but-not-clicked samples are not available to the model, \textit{Reciprocal Ratio Negative Sampling} is a good protocol that enhances the quality of negative samples.
% produced by commonly-used sampling strategies.

\subsubsection{Effects of Meta Preferences}
\label{sec:experiments:meta_preferences}



\begin{figure}
\centering     %%% not \center

\subfigure[Model performance varies with the number of meta-preferences. Best performance is obtained at $N_m=64$.]{\label{fig:effects_of_meta_preference}\includegraphics[width=0.48\linewidth]{content/figures/meta_preferences_compare.png}}
\hfill
\subfigure[Model performance varies with the ratio $\epsilon$ of Soft Distance Correlation.
$\epsilon=0$ trains preference embeddings without Distance Correlation Loss; $\epsilon=1$ reduces to Distance Correlation.
]{\label{fig:effects_of_soft_distance_correlation}\includegraphics[width=0.48\linewidth]{content/figures/PCA_compare.png}}
\vspace{-0.5cm}
\caption{Hyperparameter evaluation with number of meta-preferences and Soft Distance Correlation.}
\label{fig:effects_hyperparameters}
\vspace{-0.5cm}
\end{figure}

% \begin{figure*}
% \centering     %%% not \center
% \begin{minipage}{0.61\textwidth}
% \caption{Benchmark results on Microsoft-Movie-Dataset. Best performance is marked in \textbf{bold}.}
% \label{tab:compare_baselines_movies}
% \centering
% % \small
% \footnotesize
% \begin{tabular}{llllllllll}
% \toprule
%                                   & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{ndcg}   & \multicolumn{3}{c}{Hit Ratio}  \\
% ~                                 & @20   & @60   & @100    & @20   & @60     & @100  & @20   & @60   & @100        \\
% \midrule
% BPRMF                                & 0.1387 &	0.1944&	0.2206&	0.0961&	0.1137&	0.1192&	0.1980&	0.2785&	0.3236
%           \\
% CKE & 0.1369&	0.1898&	0.2150&	0.0940&	0.1108&	0.1160&	0.1950&	0.2707&	0.3155
% \\
% KGAT&	\underline{0.1403}&	0.1928&	0.2185&	\underline{0.1006}&	0.1173&	0.1226&	0.1997&	0.2742&	0.3196
% \\
% KGIN&	0.1351&	\underline{0.2119}&	\underline{0.2445}&	0.0982&	\underline{0.1254}&	\underline{0.1322}&	\underline{0.2194}&	\underline{0.3081}&	\underline{0.3643}\\

% \midrule
% KMPN & 0.1434&	0.2130&	0.2427&	0.1073&	0.1305&	0.1367&	0.2193&	0.3098&	0.3602
% \\
% NRMS-BERT& 0.0941&	0.1456&	0.1598&	0.0754&	0.0914&	0.0945&	0.1541 & 0.2034&	0.2348
% \\
% CKMPN & \textbf{0.1463}&	\textbf{0.2153}&	\textbf{0.2467}&	\textbf{0.1087}&	\textbf{0.1334}&	\textbf{0.1402}&	\textbf{0.2211}&	\textbf{0.3124}&	\textbf{0.3657}
% \\



% \bottomrule
% \end{tabular}
% \end{minipage}
% \hfill
% \begin{minipage}{0.37\textwidth}
% \subfigure[]{\label{fig:effects_of_meta_preference}\includegraphics[width=0.49\linewidth]{content/figures/meta_preferences_compare.png}}
% \subfigure[]{\label{fig:effects_of_soft_distance_correlation}\includegraphics[width=0.49\linewidth]{content/figures/PCA_compare.png}}
% \caption{Hyperparameter evaluation with number of meta-preferences and Soft Distance Correlation.}
% \label{fig:effects_hyperparameters}
% \end{minipage}
% \end{figure*}

An obvious research question is how the design of modelling user through meta-preferences improves the model performance.

As shown in Fig.~\ref{fig:effects_of_meta_preference}, $N_m=16$ achieved worse performance than $N_m\geq32$ due to the limited capacity of modelling user preference.
Peaking at $N_m=64$, the performance started to decrease at $N_m\geq128$, which suggests that bringing too many preference bridges induces overfitting and will not further improve the system, and a moderate $N_m$ is suificient for best performance.


% $\epsilon=0$ is the model where all preference embeddings $\{\bbe_{p}\in \bbR^{h}|p\in \ccalP \}$ are directly trainable instead of a distribution over meta-preferences.


\subsubsection{Effects of Soft Distance Correlation Loss}
\label{sec:experiments:soft_distance_correlation}
The hyperparameter $\epsilon$ controls the number of primary components to keep after PCA dimension reduction.
The lower the ratio, the more flexibility the preference embeddings will recover in dimensions from the standard Distance Correlation constraint.
$\epsilon=0$ removes the Soft Distance Correlation Constraint on preference embeddings completely, while $\epsilon=1$ reduces to a standard Distance Correlation Loss. 
As shown in Fig.~\ref{fig:effects_of_soft_distance_correlation},
the model performance peaks at $\epsilon = 0.5$, where half of $h$ dimensions are relaxed from the Distance Correlation constraint, and preference embeddings are still able to grow diversely in the remaining half dimensions.
As $\epsilon$ approaches 0, the Distance Correlation constraint becomes too loose to encourage the diversity of preferences, leading to a dramatically decreased performance.

\subsubsection{Effects of Cross-System Contrastive Learning}
\label{sec:experiments:cross_system_learning}
\begin{figure}
\centering     %%% not \center
\subfigure[Recall@20 (blue) and ndcg @20 (red)
]{\label{fig:effects_of_cs_loss_20}\includegraphics[width=0.48\linewidth]{content/figures/cs_loss_@20.png}}
\hfill
\subfigure[Recall@100 (blue) and ndcg @100 (red)]{\label{fig:effects_of_cs_loss_100}\includegraphics[width=0.48\linewidth]{content/figures/cs_loss_@100.png}}
\vspace{-0.5cm}
\caption{System performance against the loss weight $\lambda_{CS}$ of Cross-System Contrastive Loss. The performance at top-$100$ (right) is greatly improved while keeping the metrics of top-$20$ (left) steady until $\lambda_{CS}>0.2$.}
\label{fig:effects_of_cs_loss}
\vspace{-0.3cm}
\end{figure}

We experimented with different $\lambda_{CS}$ in order to find the best configuration for the Cross-System Contrastive Loss.
As shown in Fig.~\ref{fig:effects_of_cs_loss_20}, the system performance of top-$20$ did not drop much until $\lambda_{CS}>0.2$. But meanwhile, Fig.~\ref{fig:effects_of_cs_loss_100} demonstrates that the performance at top-$100$ increases dramatically at $\lambda_{CS}\leq 0.2$ compared to the system without the Cross-System Contrastive Loss.

Therefore, we can easily conclude that by contrastively learning cross-system user/item representations around proxies that provide anchors, CKMPN successfully fuses the external information from a content-based system, NRMS-BERT, and the improvement on all @60/@100 metrics over KMPN arises from the mutual context-aware features learned from both systems.
It is also worth noting that this contrastive learning loss is not only limited to fusing textual modality, but can be applied to any other modalities that provide already good item/user representations for recommendation.
% after proper supervised training.


% \begin{table*}[!ht]
% \caption{Benchmark results on Microsoft-Movie-Dataset. Best performance is marked in \textbf{bold}.
% }
% \label{tab:compare_baselines_movies}
% \centering
% \begin{tabular}{llllllllll}
% \toprule
%                                   & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{ndcg}   & \multicolumn{3}{c}{Hit Ratio}  \\
% ~                                 & @20   & @60   & @100    & @20   & @60     & @100  & @20   & @60   & @100        \\
% \midrule
% BPRMF                                & 0.1699&	0.2063&	0.2251&	0.1458&	0.1577&	0.1616&	0.2169&	0.2724&	0.3082

%           \\
% CKE & 0.1708&	0.2114&	0.2333&	0.1407&	0.1536&	0.1582&	0.2195&	0.2832&	0.3240\\
% KGAT&	0.1857&	0.2347&	0.2630&	0.1562&	0.1708&	0.1767&	0.2465&	0.3244&	0.3739\\
% KGIN&	0.1968&	0.2525&	0.2818&	0.1595&	0.1762&	0.1823&	0.2680&	0.3522&	0.4022\\
% \midrule
% KMPN & \textbf{0.2006}&	0.2539&	0.2827&	0.1618&	\textbf{0.1781}&	0.1841&	0.2696&	0.3538&	0.4033\\
% NRMS-BERT&0.1482&	0.1880&	0.2068&	0.1227&	0.1369&	0.1407&	0.2066&	0.2603&	0.2953
% \\
% CKMPN & 0.1999 &	\textbf{0.2545}&	\textbf{0.2836}&	\textbf{0.1619}&	0.1779&	\textbf{0.1842}&	\textbf{0.2699}&	\textbf{0.3555}&	\textbf{0.4050}\\



% \bottomrule
% \end{tabular}

% \end{table*}

\subsection{Benchmarking on Microsoft-Movie-Dataset}

After verifying the effectiveness of our proposed models in Amazon-Book-Extended, we report their best performance on the newly collected movie dataset (Standard version with 19 days).\footnote{Extended version (39 days) will be released upon publication for larger applications.}
The performance of the same baseline systems is provided for inclusion (Table ~\ref{tab:compare_baselines_movies}).
The same performance boost is observed on KMPN over baselines.
CKMPN also achieved the best performance with the content-based features from NRMS-BERT.
We can conclude that our method is generalizable in different datasets.

==> content/backup/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Collaborative-filtering (CF) and content-based filtering (CBF) are two primary recommendation techniques distinguished by former work \cite{takacs2009scalable}.
The nature of two methods accounts for their application fields.
CBF models leverage only descriptive attributes of items/users and the interaction behavior of users is characterized by the content information available in the items~\cite{thorat2015survey}.
Owing to their ability in content-based user/item characterization, they are of the essence for news recommendation, with millions of new items being produced and put in recommender systems every day.
In contrast, CF method utilizes the collaborative power of the interactions provided by users in order to leverage inter-item, inter-user, or user-item dependencies to make recommendation.
It follows an underlying notion that users who interacted with a similar set of items are more likely to share preferences for other items.
Therefore, they are more popular for the recommendation of relatively static items that grow slowly in quantity, e.g., movie and book recommendation that we investigate in this paper.



The current research trend in movie/book recommendation is to develop knowledge-aware CF models grounded on knowledge graphs (KGs) that have showed a great potential in fusing domain knowledge or common knowledge into traditional CF recommendation.
These KG-based CF models normally map items to KG entities in order that items can exchange features with KG entities in a structure-aware manner~\cite{wang2021learning, wang2019kgat}.

However, though KG-based CF models have achieved a good performance, content-based information of items and users remains unexploited.
Recent years have witnessed the fast evolution and excellent performance of large pre-trained transformer models for language understanding, such as BERT~\cite{devlin-etal-2019-bert} and GPT-2~\cite{radford2019language}.
We note that combining transformers in KG-based CF models may improve the overall system performance with more powerful contextual embeddings, but related research is still missing.
Attempts have been made to fuse content-based features into CF models, but these features were mostly derived from unsupervised methods.
For example, CKE~\cite{zhang2016collaborative} utilizes an unsupervised deep learning model called stacked denoising auto-encoders (S-DAE) to get items’ textual representations from texts and incorporate them in collaborative filtering.
The challenge of combining a transformer with KG-based CF models mainly stems from the necessity of co-occurrence of graph node features - 
graph convolution grounded on KGs requires the representations of graph nodes to be back-propagated and updated after each forward pass, which is prohibited in large graphs where million-scale nodes need transformer-generated embeddings.


Therefore, this paper aims to investigate towards an efficient approach to leverage transformer-based content-aware features in knowledge-graph-enhanced collaborative filtering.
We introduced a fusion framework that incorporates transformer-generated content-based features in CF training.
To obtain the best performance, we firstly presented a powerful CF model, Knowledge-Graph-Enhanced Meta-Preference Network (KMPN), which leverages meta-preferences to build user-item preference bridges and outperformed some existing baseline models.
We then upgraded a famous content-based model - Neural Recommendation with Multi-head Self-attention (NRMS)~\cite{wu-etal-2019-neural-news} - to exploit a pre-trained transformer and extract content-based embeddings from movie/book descriptions.
% to exploit the powerful pre-trained BERT model \cite{devlin-etal-2019-bert} for extracting content-based features for users and items.
% Finally, a fusion framework, Content-Aware KMPN (CKMPN), that incorporates pre-trained content-based features as target for cross-system contrastive learning is proposed to reach the best performance.
Finally, Content-based KMPN (CKMPN) fuses the information of two systems with cross-system contrastive learning while the training cost and inference complexity of KMPN is preserved.

In the meanwhile, new datasets dedicated for such an investigation are in great need, as multi-modal datasets that consist of (1) large-scale user-item interactions, (2) up-to-date enormous knowledge graphs for tasks, and (3) rich descriptive attributes that are suitable for content-based movie/book recommendation, is still missing.
To facilitate the domain research, we extended the popular Amazon-Book dataset with summary texts for books and prepared a large-scale movie recommendation dataset that satisfies the growing need of the research community.

Our contributions are summarized as follows:

(1) 
% For investigating content-aware CF recommendation, 
We extended the popular book recommendation dataset Amazon-Book, and further collected a brand-new large-scale dataset for movie recommendation.

(2) We demonstrated the benefits of merging content-based feature into CF training by proposing a fusion framework with the cross-system contrastive learning. 
To support the framework, a powerful CF model (KMPN) and a transformer-augmented CBF model (NRMS-BERT) were introduced and evaluated.

(3) Based on two real-world datasets, extensive experiments were conducted to evaluate the effectiveness of our proposed models.
We further provide benchmarking results for the newly-collected million-scale dataset which will be shared upon publication.
% (1) For investigating content-aware CF recommendation, we extended the popular book recommendation dataset Amazon-Book, and further collected a brand-new large-scale dataset for movie recommendation.

% (2) We proposed a CF-based model that outperformed several existing baselines with Meta-Preference Modelling and Reciprocal Ratio Negative Sampling.

% (3) We introduced a fusion framework that leverages transformer-generated content-based features extracted by NRMS system as cross-system contrastive targets, and achieved improvements over the baselines.

% (4) Based on two real-world datasets, extensive experiments were conducted to evaluate the effectiveness of our proposed models.
% On top of this, we provide benchmarking results for the newly-collected million-scale dataset which will be shared upon publication.

Finally, though conducting extensive experiments with our proposed model, we emphasize that our aim is to pioneer the research direction of content-aware KG-based CF recommendation and show its potential by providing high quality datasets and strong models for benchmarking.

% Beyond these two methods is a hybrid approach for recommendation, which aims to leverage the advantages of either model.


% This paper focuses on the exploration of fusing  with deep learning approach.


==> content/backup/methodology.tex <==
\section{Methodology}
\begin{figure*}
\centering
\includegraphics[width=0.8\linewidth]{content/figures/new_pipeline.drawio.png}
\vspace{-0.4cm}
\caption{Framework pipeline. (1) KMPN: leverages meta preferences to model users from knowledge graph entities and interacted items; (2) Soft Distance Correlation: encourage preference bridges to separate at low dimensions; (3) NRMS-BERT: extracts content-based features; (4) Cross System Contrastive Learning: encourages user/item embeddings to learn mutual information from content-based representations;
(5) Rating: uses dot product of KMPN user/item features.}
\vspace{-0.3cm}
\end{figure*}
In this section, we first introduce notations and data structures (Sec.~\ref{sec:data_structure}).
We then propose a CF model that serves as a strong base model (Sec.~\ref{sec:cf_model}), and then move on to propose a content-based model that rates items through a transformer with rich texts provided by our datasets (Sec.~\ref{sec:cbf_model}).
Finally, built on top of these two strong models, we introduce a simple fusion framework that leverages the information provided by each while preserving the CF model as the framework backbone (Sec.~\ref{sec:merge_model}).

\subsection{Structured and Unstructured Data}
\label{sec:data_structure}
There are $N_u$ users $\{u| u \in \mathcal{S}_u\}$ and $N_i$ items $\{i|i \in \mathcal{S}_i\}$.
$\mathcal{P}^{+}=\{(u, i) | u\in \mathcal{S}_u, i \in \mathcal{S}_i\}$ is the set of user interactions. Each $(u, i)$ pair indicates user $u$ interacted with $i$.
Each item $i \in \mathcal{S}_i$ carries unstructured data $\bbx_i$, e.g., a text description of the item.

The knowledge graph (thereafter KG) contains structured information that describes relations between real world entities. 
It can be represented by a weighted heterogeneous graph defined as
$\ccalG = (\ccalV, \ccalE)$ with a node set $\ccalV$ consisting of $N_v$ nodes $\{v\}$,
and an edge set $\ccalE$ containing all edges between nodes.
The graph is also associated with a relation type mapping function $\phi:\ccalE \rightarrow \ccalR$ that maps each edge to a type in the relation set $\ccalR$ consisting of $N_r$ relations.
Note that all items are included in the KG: $\ccalS_i \subset \ccalV$.

The edges of the knowledge graph are further described by triplets $\ccalT=\{(h, r, t)|h,t\in \ccalV, r\in \ccalR\}$, where $\ccalV$ is the collection of graph entities/nodes and $\ccalR$ is the relation set.
Each triplet describes that a head entity $h$ is connected to a tail entity $t$ with the relation $r$. For example, $(The\ Shinning, film.film.actor, Jack\ Nicholson)$ describes that Jack Nicholson is an actor of the movie ``The shinning''.
To fully exploit the relationships between heads and tails, the relation set is extended with reversed relation types, i.e., for any $(h, r, t)$ triplet we allows inverse connection $(t, r', h)$ to be built, where $r'$ is the reverse of $r$. As a result, the edge set $\ccalE$ is derived from the triplets.

% We thus define an $N\times N$ binary adjacency matrix $\bbS$, where $[\bbS]_{ij}  = 0$ if $(v_{i}, v_{j}) \notin \ccalE$ and $1$ otherwise.



\input{content/model_cf}
\input{content/model_cbf}
\input{content/model_merge}

==> content/backup/model_cbf.tex <==
\subsection{Neural Recommendation with Multi-Head Self-Attention enhanced by BERT}
\label{sec:cbf_model}
Inspired by NRMS \cite{wu-etal-2019-neural-news}, a powerful content-based system that exhibited outstanding performance in news recommendation,
we propose a variant of NRMS, \textbf{NRMS-BERT}, that further utilizes a pre-trained transformer for extracting contextual information from descriptions of items.

The model consists of an item encoder and a user encoder.
Instead of training self-attention blocks from scratch as did in NRMS, NRMS-BERT incorporates a pretrained BERT as the base block for language understanding.

\subsubsection{Item Encoder}
The item encoder encodes the text description string $\bbx_i$ of any item $i\in \ccalS_i$ through a BERT into embeddings of size $h$ by extracting the embeddings of \texttt{<CLS>} at the last layer:
$$
\bbe_i = \mathcal{BERT}(\bbx_i) \in \bbR^h
$$

For each user, the item encoder encodes one positive item $\bbe_{i^{+}}$ and $K$ negative items $\bbe_{i^{-}_1}$, ..., $\bbe_{i^{-}_{K}}$.
$B$ items are randomly sampled from the user's browsed items $i_{u,1}$,...,$i_{u,B}$.
These browsed items are encoded and gathered to $\bbE_u = [\bbe_{i_{u,1}},...,\bbe_{i_{u,B}}] \in \bbR^{B \times h}$.
\subsubsection{User Encoder}
The user encoder leverages users' interacted items to produce a content-aware user representation.
The final user representation is a weighted sum of the $B$ browsed items:
$$
\bbe_u = \sum_{b=1}^{B} \alpha_{b} \bbe_{i_{u,b}},
$$
where $\alpha_b$ is the attention weight assigned to $i_{u,b}$ that is obtained by passing features through two linear layers:
$$
\alpha_b = \frac{\exp{(\hat{\bbA}_b)}}{\sum_{b'=1,..,B}\exp{(\hat{\bbA}_{b'})}};
$$
$$
\hat{\bbA} = \tanh(\bbE_u \bbA_{fc_1}+\bbb_{fc_1})\bbA_{fc_2}+\bbb_{fc_2} \in \bbR^{B \times 1},
$$
where $\bbA_{fc_1} \in \bbR^{h\times \frac{1}{2}h}$, $\bbb_{fc_1} \in \bbR^{\frac{1}{2}h}$, $\bbA_{fc_2} \in \bbR^{\frac{1}{2}h\times 1}$, and $\bbb_{fc_2} \in \bbR^{1}$ are weights and biases of two fully-connected layers, respectively.

\subsubsection{Model Optimization}
% Having modelled the representations of users from their interacted items, 
The rating is the dot product of user and item embeddings:
$
\hat{y}_{ui} = (\bbe_u)^\mathsf{T} \cdot \bbe_i.
$
Assume that the scores of the positive samples and negative samples are $\hat{y}^{+}$ and $\hat{y}^{-}_{1}$,...,$\hat{y}^{-}_{K}$, following \cite{wu-etal-2019-neural-news}, the loss for optimization is the log posterior click probability of item $i$:
$$
\ccalL_{NRMS} = -\sum_{i \in \ccalS_i} \log{(\frac{\exp{(\hat{y}^{+})}}{\hat{y}^{+}+\sum_{k=1,..,K}\exp{(\hat{y}^{-}_{k})}})}
$$

==> content/backup/model_cf.tex <==
\subsection{Knolwedge-Graph-Enhanced Meta-Preference Network}
\label{sec:cf_model}
In this subsection, we introduce Knolwedge-graph-enhanced Meta-Preference Network (thereafter KMPN), a collaborative filtering model.
It firstly aggregates features of all KG entities to items efficiently with the help of KG, and then fuses item features over preference bridges to users for preference-aware recommendation.

\subsubsection{Gated Path Graph Convolution Networks}

% We define an $N_v\times N_v$ binary symmetric adjacency matrix $\bbS$, where $[\bbS]_{ij}  = 0$ if $(v_{i},v_{j}) \notin \ccalE$ and $1$ otherwise.
% Associated with each KG node $v_i$ are feature vectors $\bbx^i \in \mathbf R^F$.
% They are gathered into matrices $\bbX$ of dimension  $N_v\times F$, where $F$ is the model's hidden size.


% % In this way $\bbS^{k} \bbX = \bbS(\bbS^{k-1}\bbX)$ is equivalent to $k$ rounds of feature exchanges with neighbours.

% A convolution layer transforms an input $\bbX \in \mathbf{R}^{N\times F}$ to an output $\mathcal G(\bbX) \in \mathbf{R}^{N\times F}$ as follows.
% Note that $\bbS\bbX$ is mathematically equivalent to passing the features of each graph node to its neighbours.
% \begin{equation}
% \label{eqn:graphAttentionConv}
% \begin{split}
%     % \ccalA(\bbX; \bbS) & = (\bbE \odot \bbS)^{k} \bbX \bbA_{k}  \\
%     \mathcal G(\bbX) &  =  \sigma \big[ (\bbE \odot \bbS) \bbX \bbA \big], 
% \end{split}
% \vspace{-0.5cm}
% \end{equation}

% where the $\{\bbA\}$ are $\mathbf{R}^{F \times F}$ linear feature transforms
% and $\sigma(.)$ is a non-linear activation function.

Associated with each KG node $v_i$ are feature vectors $\bbe_i^{(0)} \in \bbR^h$.
Each relation type $r \in \ccalR$ is also associated with a relational embedding $\bbe_r$.
The Gated Path Graph Convolution Networks are a cascade of $L$ convolution layers.
For each KG node, a convolution layer aggregates features from its neighbors as follows:
$$
\bbe_i^{(l+1)} = \frac{1}{|\ccalN_i|} \sum_{\{v_j|(v_i, r_{ij}, v_j) \in \ccalT\}} \gamma_{ij} \bbe_{r_{ij}} \odot \bbe_j^{(l)},
$$
where the neighbouring set of $i$: $\ccalN_i=\{v_j|(v_i, r_{ij}, v_j) \in \ccalT\}$, $r_{ij}$ is the type of relation from $v_i$ to $v_j$, and $\gamma_{ij}$ is a gated function that controls messages that flows from $v_j$ to $v_i$:
$$
\gamma_{ij} = \sigma(\bbe_i ^\mathsf{T} \bbe_{r_{ij}}),
$$
where $\sigma(.)$ is a sigmoid function that limits the gated value between $0$ and $1$.

% transforms an input $\bbX \in \mathbf{R}^{N_v\times F}$ to an output $\mathcal G(\bbX) \in \mathbf{R}^{N_v\times F}$ as follows.

As a result, the message passed to a node will be weighted by its importance to the node of arrival and the relation type.
% The feature at a node $v_j$ is passed through a gate to reach $v_i$ with a gated value controlling how useful this feature is to $v_i$.
Through stacking multiple layers of convolution, the final embedding at a node is aware of the path through which the features undergo and the importance of messages is considered.

To overcome the over-smooth issue of graph convolutions, the embedding at a KG node after $l$ convolutions is an aggregation of all the intermediate output embeddings:
$
\bbe_i^{l} = \sum_{l'=0}^{l}\bbe_i^{(l')}. 
$
\subsubsection{User Preference Bridges}
Inspired by \citet{wang2021learning}, we model users using a combination of preferences.

\citet{wang2021learning} assumed that each user is influenced by multiple intents and each intent is a diverse consideration over multiple movie attributes, such as the combination of the two relation types $film.film.director$ and $film.film.genre$.
Based on this assumption, they proposed to aggregate item embeddings to users through ``preferences''.
Each preference is a linear combination of all edge relation types, representing users' latent intents over different relationships in KG:
$$
\bbe_p=\sum_{r\in \ccalR} \alpha_{rp} \bbe_r,
$$
where $\alpha_{rp}$ is a Softmax-ed trainable weight.
% , for example, $\bbe_p$ can be $0.13\bbe_{r_{1}} + 0.38\bbe_{r_{2}} + 0.49\bbe_{r_{3}}$.

However, we argue that users' preferences are not only limited to spread over relations, but can be extended to more general cases.
We model each preference through a combination of meta-preferences.
Each meta-preference (``stone'') $m \in \ccalM$ is associated with a trainable embedding $\bbe_m \in \bbR^{h}$, and a preference ``bridge'' $p \in \ccalP$ is formed by different compositions of these ``stones'' as follows:
$$
\bbe_p=\sum_{m\in \ccalM} \beta_{pm} \bbe_m,
$$
where $\ccalP$ is the collection of all $N_p$ preferences, and the linear weights $\{\beta_{pm}|m \in \ccalM\}$ is derived from trainable weights $\{\hat{\beta}_{pm}|m \in \ccalM\}$ for each preference $p$:
$$
\beta_{pm} = \frac{\exp{(\hat{\beta}_{pm})}}{\sum_{m'\in \ccalM}\exp{(\hat{\beta}_{pm'})}}
$$

As a result, meta-preferences are trained to be more general interest of all users.
The user can now be profiled by passing the embeddings of interacted items through these preference ``bridges'':
$$
\bbe_u^{(l)} = \sum_{p\in \ccalP} \alpha_p \sum_{(u,i) \in \ccalP^{+}} \bbe_i^{(l)} \odot \bbe_p,
$$
where $\alpha_p$ is an attention mechanism that weights the interest of users over different preferences:
$$
\alpha_p = \frac{\exp{(\bbe_p ^\mathsf{T} \bbe_u)}}{\sum_{p'\in \ccalP}\exp{(\bbe_{p'} ^\mathsf{T} \bbe_u)}}.
$$ 

In summary, each preference is a combination of general and diverse meta-preferences, which enhances the expressiveness of preferences.
Users are further profiled by multiple preferences which focus on different aspects of item features in the KG, leading to preference-aware user-specific embeddings for recommendation.

Similar to items, the final user embedding is:
$
\bbe_u^{l} = \sum_{l'=0}^{l}\bbe_u^{(l')}.
$
\subsubsection{Soft Distance Correlation for Training Preferences}
Having modelled users through preference bridges, \citet{wang2021learning} proposed to add an additional loss that utilizes Distance Correlation (DCorr) to separate the representations of these learnt preferences as much as possible, in order to obtain differentiable proxies bridging users and items.
% $$
% \ccalL_{DCorr} = \sum_{p,p'\in \ccalP, p\neq p'} DCor(\bbe_p, \bbe_{p'}),
% $$
% where the $DCorr$ distance correlation function measures or both linear and non-linear dependencies between two variables:
% $$
% DCor(\bbe_p, \bbe_{p'}) = \frac{DCov(\bbe_p, \bbe_{p'})}{\sqrt{DVar(\bbe_p) \cdot  DVar(\bbe_{p'})}},
% $$
% where $DCov(\cdot)$ computes distance covariance of two preference embeddings and $DVar(\cdot)$ measures distance variance of a representation.
Though the authors proved that this design achieved a considerable improvement over baselines, we argue that applying constraints to all dimensions of preference embeddings leads to less flexibility in their expressiveness, as they are trained to be very dissimilar and have diverse orientations in latent space.

We propose to adopt a more soft manner: \textbf{Soft Distance Correlation Loss}, which firstly lowers the dimensionality of preference embeddings with \textit{Primary Component Analysis} (PCA) while keeping the most differentiable features in embeddings, and then applies distance correlation constraints to encourage diverse expression in lower dimensions:
$$
\hat{\bbe}_p = \mathcal{PCA}(\{\bbe_{p'}|p'\in \ccalP \}) \in \bbR^{h\epsilon};
$$
$$
\ccalL_{SoftDCorr} = \sum_{p,p'\in \ccalP, p\neq p'} \frac{DCov(\hat{\bbe}_p, \hat{\bbe}_{p'})}{\sqrt{DVar(\hat{\bbe}_p) \cdot  DVar(\hat{\bbe}_{p'})}}.
$$
% $$
% \ccalL_{SoftDCorr} = \sum_{p,p'\in \ccalP, p\neq p'} DCor(\hat{\bbe}_p, \hat{\bbe}_{p'})
% $$
% $$
% DCor(\bbe_p, \bbe_{p'}) = \frac{DCov(\bbe_p, \bbe_{p'})}{\sqrt{DVar(\bbe_p) \cdot  DVar(\bbe_{p'})}}.
% $$
where $DCov(\cdot)$ computes distance covariance while $DVar(\cdot)$ measures distance variance.
$\epsilon$ is the ratio of primary components to keep, and \textbf{note that} $\epsilon=1$ reduces to the standard Distance Correlation Loss.
Through encouraging diverse expression at only lower dimensions, preferences have retained the flexibility in higher dimensions.
% Experiments have been done to verify this design in Sec.~\ref{sec:experiments:soft_distance_correlation}.


\subsubsection{Model Optimization with Reciprocal Ratio Negative Sampling}

To rate items, dot product between user and item embeddings is performed:
$
\hat{y}_{ui} = (\bbe_u^{L})^\mathsf{T} \cdot \bbe_i^{L}.
$


Both datasets we use do not provide hard negative samples that have been viewed by users but were not interacted with.
The common practice is to randomly sample from users' unobserved counterparts $\ccalP^{-}=\{(u, i^{-})|(u, i^{-}) \notin \ccalP^{+}\}$.
However, we notice that an item is not necessarily ``not interesting'' to a user if no interaction happens, as not all items have been viewed by users.
We therefore propose to adopt \textit{Reciprocal Ratio Negative Sampling}, where items with more user interactions are considered popular and are sampled less frequently based on the assumption that popular items are less likely to be hard negative samples for any user.
The sampling distribution is given by a normalized reciprocal ratio of item interactions:
$$
i^{-} \sim P(i) = \frac{\frac{1}{c(i)}}{\sum_{i'\in \bbS_i}\frac{1}{c(i')}};
$$
% $$
% R(i) = \frac{1}{c(i)},
% $$
where $c(\cdot)$ counts the interactions of all users with $i$.

The training set therefore consists of positive and negative samples: $\ccalU = \{(u, i^{+}, i^{-})|(u, i^{+}) \in \ccalP^{+}, (u, i^{-}) \in \ccalP^{-}\}$.
Pairwise BPR loss is adopted to train the model, which exploits a contrastive learning concept to assign higher scores to users' historical items than those items that users are not interested in.
$$
\ccalL_{BPR}=\sum_{(u, i^{+}, i^{-})\in \ccalU} -\ln (\sigma(\hat{y}_{ui^{+}}-\hat{y}_{ui^{-}}))
$$
Together with commonly-used embedding l2 regularization and Soft Distance Correlation loss, the final loss is given by:
\begin{equation}
    \ccalL_{KMPN} = \ccalL_{BPR} + \lambda_{1} \frac{1}{2}||\Theta||_2^2 + \lambda_{2}\ccalL_{SoftDCorr},
\label{eqn:cf_loss}
\end{equation}
where $\Theta=\{\bbe_u^L, \bbe_{i^{+}}^L, \bbe_{i^{-}}^L|(u, i^{+}, i^{-})\in \ccalU \}$, and $||\Theta||_2^2$ is the L2-norm of user/item embeddings. $\lambda_1$ and $\lambda_2$ are hyperparameters that control loss weights.







==> content/backup/model_merge.tex <==
\subsection{Fusion of CF and CBF: Content-Aware KMPN}
\label{sec:merge_model}
To fuse the information from a CBF model (NRMS-BERT) to a CF model (KMPN), the difficulty arises from the inconsistency of two models.
Co-optimizing two models by merging their output embeddings is an appealing idea, but however, this is not promising:

(1) KMPN requires much more epochs to converge than NRMS-BERT, though the cost per epoch of KMPN is significantly less.
This inconsistency in convergence leans the model's expressiveness to NRMS-BERT, leading to a decreased performance compared to KMPN alone in our preliminary experiments.

(2) CBF models that utilize large transformers can not be co-optimized with KG-based CF models, as graph convolution requires all embeddings to be present before convolution and this requires enormous GPU memory for even one single forward pass.

(3) Fusing pre-trained features from two models did not perform any better since the user/item representations has been determined in prior supervised training. Applying traditional aggregation methods (e.g., concatenation, MLP layers, multi-head attention) to combine features from two distinct systems broke the already-learned expressiveness and therefore showed worse performance in our preliminary experiments.

Therefore, a better way to fuse features is required, in line with three principles to make training efficient: (1) not optimizing two models together; (2) fusing features without learning towards the expressiveness of NRMS-BERT (3) not applying traditional feature aggregation on pre-trained embeddings.

Here, in line with our expectation to use a CF model for movie/book recommendation, we present a novel and efficient approach of fusing information for training a better KMPN: \textit{Cross-System Contrastive Learning}.
KMPN is still used as the framework backbone, and it is trained with the aid of a pre-trained NRMS-BERT.

In KMPN training,
for user and item in $(u, i^{+}, i^{-})\in \ccalU$,
embeddings are generated from NRMS-BERT: $e_u^{NRMS}$, $e_{i^{+}}^{NRMS}$, $e_{i^{-}}^{NRMS}$, and from KMPN: $e_u^{KMPN}$, $e_{i^{+}}^{KMPN}$, and $e_{i^{-}}^{KMPN}$.

\textit{Cross-System Contrastive Loss} is adopted to encourage KMPN system learns to incorporate content-aware features from NRMS-BERT features:
\begin{equation}
\begin{aligned}
    \ccalL_{CS}=\sum_{(u, i^{+}, i^{-})\in \ccalU} &-\ln \Big (\sigma \big ((\bbe_u^{KMPN})^\mathsf{T} \cdot \bbe_{i^{+}}^{NRMS}-(\bbe_u^{KMPN})^\mathsf{T} \cdot \bbe_{i^{-}}^{NRMS}\big) \Big) \\
    &-\ln \Big (\sigma \big ((\bbe_u^{NRMS})^\mathsf{T} \cdot \bbe_{i^{+}}^{KMPN}-(\bbe_u^{NRMS})^\mathsf{T} \cdot \bbe_{i^{-}}^{KMPN}\big) \Big)
\end{aligned}
\label{eqn:cross_system_loss}
\end{equation}

This loss encourages KMPN to produce item embeddings that can not only interact with its own user embeddings, but also with NRMS-BERT's user embeddings.
Similarly, user embeddings of KMPN are trained to interact with items of NRMS-BERT.
It allows $\bbe_i^{KMPN}$ to learn mutual expressiveness with $\bbe_i^{NRMS}$, but without approaching the two embeddings directly using similarity (e.g. cosine-similarity), which has been proved to damage the performance in experiments.
In this case, $\bbe_u^{NRMS}$ serves as a bridge with which the item embeddings of two systems learn to share commons and increase their mutuality.

A more mathematical explanation states that this loss encourages $\bbe_i^{KMPN}$ and $\bbe_i^{NRMS}$ to lie in the same hidden space hyperplane on which features have the same dot-product results with $\bbe_u^{NRMS}$.
This contrastive constraint optimizes KMPN to grow embeddings in the same region of hidden space, leading to mutual experessiveness across two systems.


Finally, the optimization target is:
$$
\ccalL_{CKMPN} = \ccalL_{KMPN} + \lambda_{CS}\ccalL_{CS},
$$
where $\lambda_{CS}$ controls the weight of the Cross-System Contrastive Loss.



% Context-Aware Knowledge-Graph-Enhanced Meta-Preference Network


==> content/backup/related_work.tex <==
\section{Related Work}
% \subsection{Recommender Systems}
% The two broad high-level categories for recommendation systems are content-based filtering (CBF) and collaborative filtering (CF).
% CBF models extracts users' preferences over items from the descriptive attributes, such as item category, title, and content~\cite{ijcai2019-0536, liu2020kred}.
% Unlike CBF models, CF models features its power to model a user collaboratively with the user-item interactions of other users.
% Among the most popular and successful CF approaches, Matrix Factorization (MF) has been developed rapidly due to the Netflix Prize Challenge in 2006-2009.
% MF models \cite{svd_plus, rendle2012bpr, paterek2007improving, rendle2013scaling, koren2009collaborative, koren2009matrix} ``factorizes'' the observed sparse user-item interaction matrix into the approximate product of two low-rank matrices which contain user and item embeddings.
% % Through learning these embeddings, user/item similarity can be computed.
% To compensate for the data sparsity and cold-start problem, Factorization Machines (FM) were proposed to incorporate arbitrary auxiliary features~\cite{10.1145/2009916.2010002, 10.1145/3077136.3080777}.
% Neural forms of FMs have also achieved a great performance in many recommendation tasks \cite{10.1145/3077136.3080777, wideanddeep, ijcai2017-0239}. 
% % For example, DeepFM~\cite{ijcai2017-0239} combines the power of FMs and deep learning for feature extraction to outperform other FM models.
% As a side note, a recent study \cite{rendle2019difficulty} showed that traditional MF methods \cite{paterek2007improving, rendle2013scaling, koren2009collaborative, koren2009matrix} are not worse than those recently proposed deep-learning-based models.


% attempt to learn low-dimensional representations, or embeddings, of users and items in a shared latent factor space. In essence, the observed sparse user-item interaction matrix is “factorized” into the approximate product of two low-rank matrices which contain user and item embeddings. After these latent factors are learned, user/item similarity can be computed and unobserved preferences inferred by comparing the user/item latent factor representations.

% \subsection{Knowledge-Graph-Enhanced Recommender Systems}

Beyond the traditional graph-based recommender systems where only user-item interactions are exploited~\cite{ying2018graph, he2020lightgcn},
recent advances in KG-based models have demonstrated the effectiveness of fusing valuable external knowledge from auxiliary KGs to improve the both accuracy and explainability of recommendation.
Below we summarize the key methods of KG-based CF models, which have been extensively investigated in recent years.

\textbf{Embedding-based Methods} rely on the underlying notion that KG head and tail entities are bridged by their first-order relations, and the relations with the same type in the KG are assumed to share the same embedding.
KG embedding methods (e.g TransE~\cite{bordes2013translating}, TransH~\cite{wang2014knowledge} and TransR~\cite{wang2016text}) are often hired to learn KG-aware entity embeddings, which are then fed into CF models for knowledge-aware recommendation~\cite{wang2019multi, zhang2016collaborative, cao2019unifying}.
For example, CKE~\cite{zhang2016collaborative} proposed to use a Bayesian formulation of TransR to extract structural representations by considering the heterogeneity of both nodes and relationships.
KTUP~\cite{cao2019unifying} jointly trained KG completion and item recommendation simultaneously with item embeddings enhanced by TransH-powered KG completion.
MKR~\cite{wang2019multi} hires ``cross\&compress'' units to associate item recommendation with the learning of KG embeddings.

\textbf{Path-based Methods} focuses on longer range connectivity in the graph. Features are aggregated from distant KG entities to users following the paths in between them~\cite{hu2018leveraging,jin2020efficient, yu2014personalized, zhao2017meta}.
For example, \citet{yu2014personalized}
and \citet{zhao2017meta} exploited manually-designed meta-paths in the heterogeneous KG to achieve path-aware feature aggregation.
However, these meta-paths are domain-specific and require domain experts for feature engineering, which is not feasible for larger KGs with enormous path types and limits its transferability to different domains.

\textbf{GNN-based Methods} aggregate features grounded on the convolution mechanism of Graph Neural Networks (GNNs)~\cite{hamilton2017inductive}, including the variants such as Graph Attention Networks (GATs)~\cite{velivckovic2017graph}.
Various systems have been proposed with the core to deliver neighboring features to the node of interest~\cite{wang2019knowledge,10.1145/3308558.3313417,jin2020efficient, wang2019kgat, wang2020ckan}.
For example, KGIN~\cite{wang2021learning} embeds relational embeddings in inter-node feature passing in order to achieve path-aware graph convolution.
However, limited by the co-occurrence issue (Sec.~\ref{sec:introduction}) and relevant datasets, the work in incoporating content-based features and leveraging transformers is still missing.

% As explained in Sec.~\ref{sec:introduction},
In contrast to CF models introduced above,
CBF models are extensively investigated in the field of news recommendation as news gets expired quickly than movies and books.
Most research of KG-based CBF focuses on enhancing the item embeddings with KG embeddings by mapping relevant KG entities to the content of items, e.g., by entity linking~\cite{liu2020kred, wang2018dkn}.
For example, DKN~\cite{wang2018dkn} fuses the word-level and knowledge-level representations of news and generate a knowledge-aware embedding vector for content-based recommendation.
However, these methods heavily rely on word-level entity mapping with common knowledge bases, which is prohibited for movie/book since their descriptions mostly consist of imaginary content, e.g., character names and fictional stories.

% \subsection{Datasets for Recommendation}

==> content/content_main.tex <==
\section{Introduction}
\label{sec:introduction}
Collaborative-filtering (CF) and content-based filtering (CBF) are two primary recommendation techniques distinguished by former work \cite{takacs2009scalable}.
The nature of two methods accounts for their application fields.
CBF models leverage only descriptive attributes of items/users and the interaction behavior of users is characterized by the content information available in the items~\cite{thorat2015survey}.
Owing to their ability in content-based user/item characterization, they are of the essence for news recommendation, with millions of new items being produced and put in recommender systems every day.
In contrast, CF method utilizes the collaborative power of the interactions provided by users in order to leverage inter-item, inter-user, or user-item dependencies to make recommendation.
It follows an underlying notion that users who interacted with a similar set of items are more likely to share preferences for other items.
Therefore, they are more popular for the recommendation of relatively static items that grow slowly in quantity, e.g., movie and book recommendation that we investigate in this paper.



The current research trend in movie/book recommendation is to develop knowledge-aware CF models grounded on knowledge graphs (KGs) that have showed a great potential in fusing domain knowledge or common knowledge into traditional CF recommendation.
These KG-based CF models normally map items to KG entities in order that items can exchange features with KG entities in a structure-aware manner~\cite{wang2021learning, wang2019kgat}.

However, though KG-based CF models have achieved a good performance, content-based information of items and users remains unexploited.
Recent years have witnessed the fast evolution and excellent performance of large pre-trained transformer models for language understanding, such as BERT~\cite{devlin-etal-2019-bert} and GPT-2~\cite{radford2019language}.
We note that combining transformers in KG-based CF models may improve the overall system performance with more powerful contextual embeddings, but related research is still missing.
Attempts have been made to fuse content-based features into CF models, but these features were mostly derived from unsupervised methods.
For example, CKE~\cite{zhang2016collaborative} utilizes an unsupervised deep learning model called stacked denoising auto-encoders (S-DAE) to get items’ textual representations from texts and incorporate them in collaborative filtering.
The challenge of combining a transformer with KG-based CF models mainly stems from the necessity of co-occurrence of graph node features - 
graph convolution grounded on KGs requires the representations of graph nodes to be back-propagated and updated after each forward pass, which is prohibited in large graphs where million-scale nodes need transformer-generated embeddings.


Therefore, this paper aims to investigate towards an efficient approach to leverage transformer-based content-aware features in knowledge-graph-enhanced collaborative filtering.
We introduced a fusion framework that incorporates transformer-generated content-based features in CF training.
To obtain the best performance, we firstly presented a powerful CF model, Knowledge-Graph-Enhanced Meta-Preference Network (KMPN), which leverages meta-preferences to build user-item preference bridges and outperformed some existing baseline models.
We then upgraded a famous content-based model - Neural Recommendation with Multi-head Self-attention (NRMS)~\cite{wu-etal-2019-neural-news} - to exploit a pre-trained transformer and extract content-based embeddings from movie/book descriptions.
% to exploit the powerful pre-trained BERT model \cite{devlin-etal-2019-bert} for extracting content-based features for users and items.
% Finally, a fusion framework, Content-Aware KMPN (CKMPN), that incorporates pre-trained content-based features as target for cross-system contrastive learning is proposed to reach the best performance.
Finally, Content-based KMPN (CKMPN) fuses the information of two systems with cross-system contrastive learning while the training cost and inference complexity of KMPN is preserved.

In the meanwhile, new datasets dedicated for such an investigation are in great need, as multi-modal datasets that consist of (1) large-scale user-item interactions, (2) up-to-date enormous knowledge graphs for tasks, and (3) rich descriptive attributes that are suitable for content-based movie/book recommendation, is still missing.
To facilitate the domain research, we extended the popular Amazon-Book dataset with summary texts for books and prepared a large-scale movie recommendation dataset that satisfies the growing need of the research community.

Our contributions are summarized as follows:

(1) 
% For investigating content-aware CF recommendation, 
We extended the popular book recommendation dataset Amazon-Book, and further collected a brand-new large-scale dataset for movie recommendation.

(2) We demonstrated the benefits of merging content-based feature into CF training by proposing a fusion framework with the cross-system contrastive learning. 
To support the framework, a powerful CF model (KMPN) and a transformer-augmented CBF model (NRMS-BERT) were introduced and evaluated.

(3) Based on two real-world datasets, extensive experiments were conducted to evaluate the effectiveness of our proposed models.
We further provide benchmarking results for the newly-collected million-scale dataset which will be shared upon publication.
% (1) For investigating content-aware CF recommendation, we extended the popular book recommendation dataset Amazon-Book, and further collected a brand-new large-scale dataset for movie recommendation.

% (2) We proposed a CF-based model that outperformed several existing baselines with Meta-Preference Modelling and Reciprocal Ratio Negative Sampling.

% (3) We introduced a fusion framework that leverages transformer-generated content-based features extracted by NRMS system as cross-system contrastive targets, and achieved improvements over the baselines.

% (4) Based on two real-world datasets, extensive experiments were conducted to evaluate the effectiveness of our proposed models.
% On top of this, we provide benchmarking results for the newly-collected million-scale dataset which will be shared upon publication.

Finally, though conducting extensive experiments with our proposed model, we emphasize that our aim is to pioneer the research direction of content-aware KG-based CF recommendation and show its potential by providing high quality datasets and strong models for benchmarking.

% Beyond these two methods is a hybrid approach for recommendation, which aims to leverage the advantages of either model.


% This paper focuses on the exploration of fusing  with deep learning approach.


\section{Related Work}
% \subsection{Recommender Systems}
% The two broad high-level categories for recommendation systems are content-based filtering (CBF) and collaborative filtering (CF).
% CBF models extracts users' preferences over items from the descriptive attributes, such as item category, title, and content~\cite{ijcai2019-0536, liu2020kred}.
% Unlike CBF models, CF models features its power to model a user collaboratively with the user-item interactions of other users.
% Among the most popular and successful CF approaches, Matrix Factorization (MF) has been developed rapidly due to the Netflix Prize Challenge in 2006-2009.
% MF models \cite{svd_plus, rendle2012bpr, paterek2007improving, rendle2013scaling, koren2009collaborative, koren2009matrix} ``factorizes'' the observed sparse user-item interaction matrix into the approximate product of two low-rank matrices which contain user and item embeddings.
% % Through learning these embeddings, user/item similarity can be computed.
% To compensate for the data sparsity and cold-start problem, Factorization Machines (FM) were proposed to incorporate arbitrary auxiliary features~\cite{10.1145/2009916.2010002, 10.1145/3077136.3080777}.
% Neural forms of FMs have also achieved a great performance in many recommendation tasks \cite{10.1145/3077136.3080777, wideanddeep, ijcai2017-0239}. 
% % For example, DeepFM~\cite{ijcai2017-0239} combines the power of FMs and deep learning for feature extraction to outperform other FM models.
% As a side note, a recent study \cite{rendle2019difficulty} showed that traditional MF methods \cite{paterek2007improving, rendle2013scaling, koren2009collaborative, koren2009matrix} are not worse than those recently proposed deep-learning-based models.


% attempt to learn low-dimensional representations, or embeddings, of users and items in a shared latent factor space. In essence, the observed sparse user-item interaction matrix is “factorized” into the approximate product of two low-rank matrices which contain user and item embeddings. After these latent factors are learned, user/item similarity can be computed and unobserved preferences inferred by comparing the user/item latent factor representations.

% \subsection{Knowledge-Graph-Enhanced Recommender Systems}

Beyond the traditional graph-based recommender systems where only user-item interactions are exploited~\cite{ying2018graph, he2020lightgcn},
recent advances in KG-based models have demonstrated the effectiveness of fusing valuable external knowledge from auxiliary KGs to improve the both accuracy and explainability of recommendation.
Below we summarize the key methods of KG-based CF models, which have been extensively investigated in recent years.

\textbf{Embedding-based Methods} rely on the underlying notion that KG head and tail entities are bridged by their first-order relations, and the relations with the same type in the KG are assumed to share the same embedding.
KG embedding methods (e.g TransE~\cite{bordes2013translating}, TransH~\cite{wang2014knowledge} and TransR~\cite{wang2016text}) are often hired to learn KG-aware entity embeddings, which are then fed into CF models for knowledge-aware recommendation~\cite{wang2019multi, zhang2016collaborative, cao2019unifying}.
For example, CKE~\cite{zhang2016collaborative} proposed to use a Bayesian formulation of TransR to extract structural representations by considering the heterogeneity of both nodes and relationships.
KTUP~\cite{cao2019unifying} jointly trained KG completion and item recommendation simultaneously with item embeddings enhanced by TransH-powered KG completion.
MKR~\cite{wang2019multi} hires ``cross\&compress'' units to associate item recommendation with the learning of KG embeddings.

\textbf{Path-based Methods} focuses on longer range connectivity in the graph. Features are aggregated from distant KG entities to users following the paths in between them~\cite{hu2018leveraging,jin2020efficient, yu2014personalized, zhao2017meta}.
For example, \citet{yu2014personalized}
and \citet{zhao2017meta} exploited manually-designed meta-paths in the heterogeneous KG to achieve path-aware feature aggregation.
However, these meta-paths are domain-specific and require domain experts for feature engineering, which is not feasible for larger KGs with enormous path types and limits its transferability to different domains.

\textbf{GNN-based Methods} aggregate features grounded on the convolution mechanism of Graph Neural Networks (GNNs)~\cite{hamilton2017inductive}, including the variants such as Graph Attention Networks (GATs)~\cite{velivckovic2017graph}.
Various systems have been proposed with the core to deliver neighboring features to the node of interest~\cite{wang2019knowledge,10.1145/3308558.3313417,jin2020efficient, wang2019kgat, wang2020ckan}.
For example, KGIN~\cite{wang2021learning} embeds relational embeddings in inter-node feature passing in order to achieve path-aware graph convolution.
However, limited by the co-occurrence issue (Sec.~\ref{sec:introduction}) and relevant datasets, the work in incoporating content-based features and leveraging transformers is still missing.

% As explained in Sec.~\ref{sec:introduction},
In contrast to CF models introduced above,
CBF models are extensively investigated in the field of news recommendation as news gets expired quickly than movies and books.
Most research of KG-based CBF focuses on enhancing the item embeddings with KG embeddings by mapping relevant KG entities to the content of items, e.g., by entity linking~\cite{liu2020kred, wang2018dkn}.
For example, DKN~\cite{wang2018dkn} fuses the word-level and knowledge-level representations of news and generate a knowledge-aware embedding vector for content-based recommendation.
However, these methods heavily rely on word-level entity mapping with common knowledge bases, which is prohibited for movie/book since their descriptions mostly consist of imaginary content, e.g., character names and fictional stories.

% \subsection{Datasets for Recommendation}

\section{Datasets}
In this section, we introduce two new datasets for recommendation: 
(1) a large-scale high-quality movie recommendation dataset that was newly collected from real user behaviors (Sec.~\ref{sec:movie_dataset});
(2) Amazon-Book-Extended dataset that derives from Amazon-Book dataset~\cite{wang2019kgat} but was newly augmented with textual book descriptions to allow the evaluation of content-based recommender systems (Sec.~\ref{sec:amazon_dataset}).

\subsection{Movie KG Dataset}
\label{sec:movie_dataset}
\subsubsection{Dataset Construction}
This dataset was formed by real user browsing behaviors that were logged by a popular commercial browser between 13/05/2021 and 20/06/2021 (39 days in total).
Sensitivity of data and privacy was firstly removed by decoupling users' real identity (e.g. IP, account identifier) from the data and assigning each user an insensitive unique virtual identifier.
To link users' browsing history with movies, we exploited an enormous commercial knowledge graph that consists of a vast number of entities and a rich set of relationships among them.
Entities with type ``movie'' were extracted together with their one-hop neighbors and edges.
As a result, a movie-specific sub-graph of Satori was ready for use.

Among billions of user browser logs, knowledge-graph entity linking was performed to match the titles of web pages with the movie titles in our refined movie-specific knowledge graph.
Movie entities were extracted using our internal service that provides NER and entity linking.

The next move is to refine user-movie interactions in order to make the dataset cleaner and more compact:
(1) Consecutive but duplicated user interactions on the same movie were merged to one single record. Browsing time (DwellTime) was aggregated.
(2) Users with less than 10 interactions in 39 days were dropped.
(3) The top frequent 50,000 movies with the most user interactions were selected.
% with the lowest user interaction count at 17.
% (3) Movies are ranked by the total amount of user interactions in 39 days, and first 50,000 movies are selected with the lowest user interaction count at 17.

After careful pre-processing and filtering, 125,218 active users with the most interactions in all days were chosen.
% They interacted with 50,000 movies in total. 
Knowledge-graph entities related to these 50,000 movies were extracted and formed a knowledge graph with 25,0327 entities (including movie items).
Each user is represented by [$UserID$, $UserHistory$], where $UserID$ is a unique identifier that has been delinked from real user identity, and $UserHistory$ is an ID list of movie items that the user has interacted with.

For training and evaluating recommender systems, $UserHistory$ was split into train/valid/test:
First 80\% of users' historical interactions (ordered by click date-time) are in the train set, 80\% to 90\% serves as the valid set, and the remaining is reserved for testing.
While validating or testing, interactions in the train set serve as users' previous clicked items and systems are evaluated on their ratings for test set items.

In addition to the traditional data split strategy, a cold-start user set was designed to help model evaluate its performance on users outside the training dataset.
3\% of users were moved to a cold-start set and they are not accessible by models at training.
This portion of interactions was split into a cold-start history set with first 80\% interactions of each user, and a test set with the remaining 20\%.



A comparison with some popular existing recommendation datasets is provided in Table~\ref{tab:comparison_with_datasets}.
\textbf{MovieLens-20M}\footnote{\href{https://grouplens.org/datasets/movielens/}{https://grouplens.org/datasets/movielens/}} is a popular benchmark that has been widely used, while
\textbf{Flixster}\footnote{\href{https://sites.google.com/view/mohsenjamali/flixter-data-set}{https://sites.google.com/view/mohsenjamali/flixter-data-set}} is large but less popular in recent work.
\textbf{Amazon-Book}~\cite{wang2019kgat}, \textbf{Last-FM}~\cite{wang2019kgat}, \textbf{Book-Crossing}~\cite{ziegler2005improving}\footnote{\href{http://www2.informatik.uni-freiburg.de/~cziegler/BX/}{http://www2.informatik.uni-freiburg.de/~cziegler/BX/}} and \textbf{Alibaba-iFashion}~\cite{wang2021learning} are dedicated for KG-based CF model evaluation.



It can be concluded that our new movie dataset consists of large-scale users and movies, and incorporates an enormous movie-specific knowledge graph with millions of triplets and entities, which has not been provided by existing popular movie recommendation datasets.
In addition, our dataset provides not only titles and genres (as in MovieLens-20M), but also other content-based information, specifically, rich summary texts of movies that enable content-based recommendation with large language understanding models (such as BERT, GPT-3).
% In addition, the dataset comprises rich texts of movie descriptions, which enable content-based recommendation with large language understanding models (such as BERT, GPT-3).


\begin{table*}[!ht]
\caption{Comparison with existing popular datasets for recommender systems.}
\label{tab:comparison_with_datasets}
\small
\begin{tabular}{llllllllll}
\toprule
Type     & Dataset                 & \#Users & \#Items & \#Interactions & Has KG? & \#Entities & \#Relations & \#Triplets & Has Descriptions?           \\ 
\midrule
% Movie    & MovieLens-25M           & 16,2000 & 62,000  & 25,000,000     & No              & N/A        & N/A         &            & No                      \\ 
Movie    & MovieLens-20M           & 138,000 & 27,000  & 20,000,000     & No              & N/A        & N/A         &    N/A        & No                      \\
Moive   & Flixster  & 1,002,796   & 66,730    & 1,048,576   & No    & N/A &   N/A & N/A & No\\
Book     & Amazon-Book             & 70,679  & 24,915  & 847,733        & Yes             & 88,572     & 39          & 2,557,746  & No                      \\ 
Book    & Book-Crossing   & 276,271   & 271,379  & 1,048,575 & Yes & 25,787 & 18 & 60,787 & No\\
Music    & Last-FM                 & 23,566  & 48,123  & 3,034,796      & Yes             & 58,266     & 9           & 464,567    & No                      \\ 
Shopping & Alibaba-iFashion        & 114,737 & 30,040  & 1,781,093      & Yes             & 59,156     & 51          & 279,155    & No                      \\
\midrule
Book     & Amazon-Book-Extended    & 70,679  & 24,915  & 847,733        & Yes             & 88,572     & 39          & 2,557,746  &  Yes       \\ 
Movie    & Movie-KG-Dataset & 125,218 & 50,000  &  4,095,146              & Yes             & 250,327    & 12          & 12,055,581 & Yes\\
\bottomrule
\end{tabular}
\vspace{-0.3cm}
\end{table*}

\subsubsection{Statistical Analysis}
\label{sec:movie_statistical_analysis}
\begin{figure}
\centering     %%% not \center
\subfigure[Length of user interactions ($\mu=32.70$,$\sigma=45.76$)]{\label{fig:hist_number_user_interactions}\includegraphics[width=0.48\linewidth]{content/figures/number_user_interactions.png}}
\hfill
\subfigure[Interactions with movies ($\mu=83.33$,$\sigma=582.50$)]{\label{fig:hist_movie_interaction_count}\includegraphics[width=0.48\linewidth]{content/figures/movie_interaction_count.png}}\\
% \subfigure[Histogram of the DwellTime of interactions]{\label{fig:hist_dwelltime}\includegraphics[width=0.48\linewidth]{content/figures/dwelltime_count.png}}
% \hfill
\subfigure[Length of texts of Movie-Dataset ($\mu=425.22$,$\sigma=329.93$)]{\label{fig:hist_movie_text_length}\includegraphics[width=0.48\linewidth]{content/figures/text_length_count_movie.png}}
\hfill
\subfigure[Length of texts of Amazon-Book-Extended ($\mu=151.75$,$\sigma=206.98$)]{\label{fig:hist_book_text_length}\includegraphics[width=0.48\linewidth]{content/figures/text_length_count_amazon.png}}
\vspace{-0.4cm}
\caption{Key statistics of Movie-KG-Dataset (Fig.~\ref{fig:hist_number_user_interactions}-\ref{fig:hist_movie_text_length}) and  Amazon-Book-Extended (Fig.~\ref{fig:hist_book_text_length}).}
\label{fig:dataset_analysis}
\vspace{-0.4cm}
\end{figure}
Fig.~\ref{tab:comparison_with_datasets} presents the key statistics of the dataset.
This dataset contains 125,218 users, 50,000 movie items, interactions. The knowledge graph contains 250,327 entities with 12 relation types and 12,055,581 triplets.
The attributes of movies include content-based properties (title, description, movie length) and properties already tied to knowledge graph entities (production company, country, language, producer, director, genre, rating, editor, writer, honors, actor).
Fig.~\ref{fig:hist_number_user_interactions}-\ref{fig:hist_movie_text_length}  show the distribution of length of interactions per user, number of interactions per movie, and length of movie descriptions respectively.
The average length of movie descriptions is 425 words, which is long enough to capture the story line of movies and infer preference.
The average number of user interactions is 32.70, providing rich resources for modelling users' long-term interest.
The first 19 days' of data (with similar data distribution but less users and interactions) is separated as ``Standard'' for most research purposes, while the full 39 days' are released as ``Extended'' for industry use.

\subsection{Extended Amazon Book Dataset}
\label{sec:amazon_dataset}
Amazon-Book dataset was originally released by ~\cite{wang2019kgat}, and was used as points for comparison of many advanced recommendation systems.
However, this dataset can not satisfy the research need as it provides only CF interaction data without content-based features for CBF evaluation.
To fill this gap, we extended the dataset with descriptions extracted from multiple data source, as the dataset was collected in 2014 and many items have expired on the Amazon website.
The procedure is summarized as below:

(1) We matched product descriptions in Amazon with entries in Amazon-Book using their unique item identifiers (asin). 24,555 items were successfully matched (98.56\%).

(2) We then matched each of the remaining item with a most relevant entry in a commercial KG such that rich descriptions were extracted. 325 items were matched at this step.

(3) The rest 28 items were matched manually to most relevant products in Amazon.

Finally, we extracted rich texts for Amazon-Book dataset with more than 99.99\% match rate, leading to an extended dataset Amazon-Book-Extended.
The distribution of description lengths is given in Fig.~\ref{fig:hist_book_text_length}, with a mean length of 151.75.

\section{Methodology}
\begin{figure*}
\centering
\includegraphics[width=0.8\linewidth]{content/figures/new_pipeline.drawio.png}
\vspace{-0.4cm}
\caption{Framework pipeline. (1) KMPN: leverages meta preferences to model users from knowledge graph entities and interacted items; (2) Soft Distance Correlation: encourage preference bridges to separate at low dimensions; (3) NRMS-BERT: extracts content-based features; (4) Cross System Contrastive Learning: encourages user/item embeddings to learn mutual information from content-based representations;
(5) Rating: uses dot product of KMPN user/item features.}
\vspace{-0.3cm}
\end{figure*}
In this section, we first introduce notations and data structures (Sec.~\ref{sec:data_structure}).
We then propose a CF model that serves as a strong base model (Sec.~\ref{sec:cf_model}), and then move on to propose a content-based model that rates items through a transformer with rich texts provided by our datasets (Sec.~\ref{sec:cbf_model}).
Finally, built on top of these two strong models, we introduce a simple fusion framework that leverages the information provided by each while preserving the CF model as the framework backbone (Sec.~\ref{sec:merge_model}).

\subsection{Structured and Unstructured Data}
\label{sec:data_structure}
There are $N_u$ users $\{u| u \in \mathcal{S}_u\}$ and $N_i$ items $\{i|i \in \mathcal{S}_i\}$.
$\mathcal{P}^{+}=\{(u, i) | u\in \mathcal{S}_u, i \in \mathcal{S}_i\}$ is the set of user interactions. Each $(u, i)$ pair indicates user $u$ interacted with $i$.
Each item $i \in \mathcal{S}_i$ carries unstructured data $\bbx_i$, e.g., a text description of the item.

The knowledge graph (thereafter KG) contains structured information that describes relations between real world entities. 
It can be represented by a weighted heterogeneous graph defined as
$\ccalG = (\ccalV, \ccalE)$ with a node set $\ccalV$ consisting of $N_v$ nodes $\{v\}$,
and an edge set $\ccalE$ containing all edges between nodes.
The graph is also associated with a relation type mapping function $\phi:\ccalE \rightarrow \ccalR$ that maps each edge to a type in the relation set $\ccalR$ consisting of $N_r$ relations.
Note that all items are included in the KG: $\ccalS_i \subset \ccalV$.

The edges of the knowledge graph are further described by triplets $\ccalT=\{(h, r, t)|h,t\in \ccalV, r\in \ccalR\}$, where $\ccalV$ is the collection of graph entities/nodes and $\ccalR$ is the relation set.
Each triplet describes that a head entity $h$ is connected to a tail entity $t$ with the relation $r$. For example, $(The\ Shinning, film.film.actor, Jack\ Nicholson)$ describes that Jack Nicholson is an actor of the movie ``The shinning''.
To fully exploit the relationships between heads and tails, the relation set is extended with reversed relation types, i.e., for any $(h, r, t)$ triplet we allows inverse connection $(t, r', h)$ to be built, where $r'$ is the reverse of $r$. As a result, the edge set $\ccalE$ is derived from the triplets.

% We thus define an $N\times N$ binary adjacency matrix $\bbS$, where $[\bbS]_{ij}  = 0$ if $(v_{i}, v_{j}) \notin \ccalE$ and $1$ otherwise.


\subsection{Knolwedge-Graph-Enhanced Meta-Preference Network}
\label{sec:cf_model}
In this subsection, we introduce Knolwedge-graph-enhanced Meta-Preference Network (thereafter KMPN), a collaborative filtering model.
It firstly aggregates features of all KG entities to items efficiently with the help of KG, and then fuses item features over preference bridges to users for preference-aware recommendation.

\subsubsection{Gated Path Graph Convolution Networks}

% We define an $N_v\times N_v$ binary symmetric adjacency matrix $\bbS$, where $[\bbS]_{ij}  = 0$ if $(v_{i},v_{j}) \notin \ccalE$ and $1$ otherwise.
% Associated with each KG node $v_i$ are feature vectors $\bbx^i \in \mathbf R^F$.
% They are gathered into matrices $\bbX$ of dimension  $N_v\times F$, where $F$ is the model's hidden size.


% % In this way $\bbS^{k} \bbX = \bbS(\bbS^{k-1}\bbX)$ is equivalent to $k$ rounds of feature exchanges with neighbours.

% A convolution layer transforms an input $\bbX \in \mathbf{R}^{N\times F}$ to an output $\mathcal G(\bbX) \in \mathbf{R}^{N\times F}$ as follows.
% Note that $\bbS\bbX$ is mathematically equivalent to passing the features of each graph node to its neighbours.
% \begin{equation}
% \label{eqn:graphAttentionConv}
% \begin{split}
%     % \ccalA(\bbX; \bbS) & = (\bbE \odot \bbS)^{k} \bbX \bbA_{k}  \\
%     \mathcal G(\bbX) &  =  \sigma \big[ (\bbE \odot \bbS) \bbX \bbA \big], 
% \end{split}
% \vspace{-0.5cm}
% \end{equation}

% where the $\{\bbA\}$ are $\mathbf{R}^{F \times F}$ linear feature transforms
% and $\sigma(.)$ is a non-linear activation function.

Associated with each KG node $v_i$ are feature vectors $\bbe_i^{(0)} \in \bbR^h$.
Each relation type $r \in \ccalR$ is also associated with a relational embedding $\bbe_r$.
The Gated Path Graph Convolution Networks are a cascade of $L$ convolution layers.
For each KG node, a convolution layer aggregates features from its neighbors as follows:
$$
\bbe_i^{(l+1)} = \frac{1}{|\ccalN_i|} \sum_{\{v_j|(v_i, r_{ij}, v_j) \in \ccalT\}} \gamma_{ij} \bbe_{r_{ij}} \odot \bbe_j^{(l)},
$$
where the neighbouring set of $i$: $\ccalN_i=\{v_j|(v_i, r_{ij}, v_j) \in \ccalT\}$, $r_{ij}$ is the type of relation from $v_i$ to $v_j$, and $\gamma_{ij}$ is a gated function that controls messages that flows from $v_j$ to $v_i$:
$$
\gamma_{ij} = \sigma(\bbe_i ^\mathsf{T} \bbe_{r_{ij}}),
$$
where $\sigma(.)$ is a sigmoid function that limits the gated value between $0$ and $1$.

% transforms an input $\bbX \in \mathbf{R}^{N_v\times F}$ to an output $\mathcal G(\bbX) \in \mathbf{R}^{N_v\times F}$ as follows.

As a result, the message passed to a node will be weighted by its importance to the node of arrival and the relation type.
% The feature at a node $v_j$ is passed through a gate to reach $v_i$ with a gated value controlling how useful this feature is to $v_i$.
Through stacking multiple layers of convolution, the final embedding at a node is aware of the path through which the features undergo and the importance of messages is considered.

To overcome the over-smooth issue of graph convolutions, the embedding at a KG node after $l$ convolutions is an aggregation of all the intermediate output embeddings:
$
\bbe_i^{l} = \sum_{l'=0}^{l}\bbe_i^{(l')}. 
$
\subsubsection{User Preference Bridges}
Inspired by \citet{wang2021learning}, we model users using a combination of preferences.

\citet{wang2021learning} assumed that each user is influenced by multiple intents and each intent is a diverse consideration over multiple movie attributes, such as the combination of the two relation types $film.film.director$ and $film.film.genre$.
Based on this assumption, they proposed to aggregate item embeddings to users through ``preferences''.
Each preference is a linear combination of all edge relation types, representing users' latent intents over different relationships in KG:
$$
\bbe_p=\sum_{r\in \ccalR} \alpha_{rp} \bbe_r,
$$
where $\alpha_{rp}$ is a Softmax-ed trainable weight.
% , for example, $\bbe_p$ can be $0.13\bbe_{r_{1}} + 0.38\bbe_{r_{2}} + 0.49\bbe_{r_{3}}$.

However, we argue that users' preferences are not only limited to spread over relations, but can be extended to more general cases.
We model each preference through a combination of meta-preferences.
Each meta-preference (``stone'') $m \in \ccalM$ is associated with a trainable embedding $\bbe_m \in \bbR^{h}$, and a preference ``bridge'' $p \in \ccalP$ is formed by different compositions of these ``stones'' as follows:
$$
\bbe_p=\sum_{m\in \ccalM} \beta_{pm} \bbe_m,
$$
where $\ccalP$ is the collection of all $N_p$ preferences, and the linear weights $\{\beta_{pm}|m \in \ccalM\}$ is derived from trainable weights $\{\hat{\beta}_{pm}|m \in \ccalM\}$ for each preference $p$:
$$
\beta_{pm} = \frac{\exp{(\hat{\beta}_{pm})}}{\sum_{m'\in \ccalM}\exp{(\hat{\beta}_{pm'})}}
$$

As a result, meta-preferences are trained to be more general interest of all users.
The user can now be profiled by passing the embeddings of interacted items through these preference ``bridges'':
$$
\bbe_u^{(l)} = \sum_{p\in \ccalP} \alpha_p \sum_{(u,i) \in \ccalP^{+}} \bbe_i^{(l)} \odot \bbe_p,
$$
where $\alpha_p$ is an attention mechanism that weights the interest of users over different preferences:
$$
\alpha_p = \frac{\exp{(\bbe_p ^\mathsf{T} \bbe_u)}}{\sum_{p'\in \ccalP}\exp{(\bbe_{p'} ^\mathsf{T} \bbe_u)}}.
$$ 

In summary, each preference is a combination of general and diverse meta-preferences, which enhances the expressiveness of preferences.
Users are further profiled by multiple preferences which focus on different aspects of item features in the KG, leading to preference-aware user-specific embeddings for recommendation.

Similar to items, the final user embedding is:
$
\bbe_u^{l} = \sum_{l'=0}^{l}\bbe_u^{(l')}.
$
\subsubsection{Soft Distance Correlation for Training Preferences}
Having modelled users through preference bridges, \citet{wang2021learning} proposed to add an additional loss that utilizes Distance Correlation (DCorr) to separate the representations of these learnt preferences as much as possible, in order to obtain differentiable proxies bridging users and items.
% $$
% \ccalL_{DCorr} = \sum_{p,p'\in \ccalP, p\neq p'} DCor(\bbe_p, \bbe_{p'}),
% $$
% where the $DCorr$ distance correlation function measures or both linear and non-linear dependencies between two variables:
% $$
% DCor(\bbe_p, \bbe_{p'}) = \frac{DCov(\bbe_p, \bbe_{p'})}{\sqrt{DVar(\bbe_p) \cdot  DVar(\bbe_{p'})}},
% $$
% where $DCov(\cdot)$ computes distance covariance of two preference embeddings and $DVar(\cdot)$ measures distance variance of a representation.
Though the authors proved that this design achieved a considerable improvement over baselines, we argue that applying constraints to all dimensions of preference embeddings leads to less flexibility in their expressiveness, as they are trained to be very dissimilar and have diverse orientations in latent space.

We propose to adopt a more soft manner: \textbf{Soft Distance Correlation Loss}, which firstly lowers the dimensionality of preference embeddings with \textit{Primary Component Analysis} (PCA) while keeping the most differentiable features in embeddings, and then applies distance correlation constraints to encourage diverse expression in lower dimensions:
$$
\hat{\bbe}_p = \mathcal{PCA}(\{\bbe_{p'}|p'\in \ccalP \}) \in \bbR^{h\epsilon};
$$
$$
\ccalL_{SoftDCorr} = \sum_{p,p'\in \ccalP, p\neq p'} \frac{DCov(\hat{\bbe}_p, \hat{\bbe}_{p'})}{\sqrt{DVar(\hat{\bbe}_p) \cdot  DVar(\hat{\bbe}_{p'})}}.
$$
% $$
% \ccalL_{SoftDCorr} = \sum_{p,p'\in \ccalP, p\neq p'} DCor(\hat{\bbe}_p, \hat{\bbe}_{p'})
% $$
% $$
% DCor(\bbe_p, \bbe_{p'}) = \frac{DCov(\bbe_p, \bbe_{p'})}{\sqrt{DVar(\bbe_p) \cdot  DVar(\bbe_{p'})}}.
% $$
where $DCov(\cdot)$ computes distance covariance while $DVar(\cdot)$ measures distance variance.
$\epsilon$ is the ratio of primary components to keep, and \textbf{note that} $\epsilon=1$ reduces to the standard Distance Correlation Loss.
Through encouraging diverse expression at only lower dimensions, preferences have retained the flexibility in higher dimensions.
% Experiments have been done to verify this design in Sec.~\ref{sec:experiments:soft_distance_correlation}.


\subsubsection{Model Optimization with Reciprocal Ratio Negative Sampling}

To rate items, dot product between user and item embeddings is performed:
$
\hat{y}_{ui} = (\bbe_u^{L})^\mathsf{T} \cdot \bbe_i^{L}.
$


Both datasets we use do not provide hard negative samples that have been viewed by users but were not interacted with.
The common practice is to randomly sample from users' unobserved counterparts $\ccalP^{-}=\{(u, i^{-})|(u, i^{-}) \notin \ccalP^{+}\}$.
However, we notice that an item is not necessarily ``not interesting'' to a user if no interaction happens, as not all items have been viewed by users.
We therefore propose to adopt \textit{Reciprocal Ratio Negative Sampling}, where items with more user interactions are considered popular and are sampled less frequently based on the assumption that popular items are less likely to be hard negative samples for any user.
The sampling distribution is given by a normalized reciprocal ratio of item interactions:
$$
i^{-} \sim P(i) = \frac{\frac{1}{c(i)}}{\sum_{i'\in \bbS_i}\frac{1}{c(i')}};
$$
% $$
% R(i) = \frac{1}{c(i)},
% $$
where $c(\cdot)$ counts the interactions of all users with $i$.

The training set therefore consists of positive and negative samples: $\ccalU = \{(u, i^{+}, i^{-})|(u, i^{+}) \in \ccalP^{+}, (u, i^{-}) \in \ccalP^{-}\}$.
Pairwise BPR loss is adopted to train the model, which exploits a contrastive learning concept to assign higher scores to users' historical items than those items that users are not interested in.
$$
\ccalL_{BPR}=\sum_{(u, i^{+}, i^{-})\in \ccalU} -\ln (\sigma(\hat{y}_{ui^{+}}-\hat{y}_{ui^{-}}))
$$
Together with commonly-used embedding l2 regularization and Soft Distance Correlation loss, the final loss is given by:
\begin{equation}
    \ccalL_{KMPN} = \ccalL_{BPR} + \lambda_{1} \frac{1}{2}||\Theta||_2^2 + \lambda_{2}\ccalL_{SoftDCorr},
\label{eqn:cf_loss}
\end{equation}
where $\Theta=\{\bbe_u^L, \bbe_{i^{+}}^L, \bbe_{i^{-}}^L|(u, i^{+}, i^{-})\in \ccalU \}$, and $||\Theta||_2^2$ is the L2-norm of user/item embeddings. $\lambda_1$ and $\lambda_2$ are hyperparameters that control loss weights.





\subsection{Neural Recommendation with Multi-Head Self-Attention enhanced by BERT}
\label{sec:cbf_model}
Inspired by NRMS \cite{wu-etal-2019-neural-news}, a powerful content-based system that exhibited outstanding performance in news recommendation,
we propose a variant of NRMS, \textbf{NRMS-BERT}, that further utilizes a pre-trained transformer for extracting contextual information from descriptions of items.

The model consists of an item encoder and a user encoder.
Instead of training self-attention blocks from scratch as did in NRMS, NRMS-BERT incorporates a pretrained BERT as the base block for language understanding.

\subsubsection{Item Encoder}
The item encoder encodes the text description string $\bbx_i$ of any item $i\in \ccalS_i$ through a BERT into embeddings of size $h$ by extracting the embeddings of \texttt{<CLS>} at the last layer:
$$
\bbe_i = \mathcal{BERT}(\bbx_i) \in \bbR^h
$$

For each user, the item encoder encodes one positive item $\bbe_{i^{+}}$ and $K$ negative items $\bbe_{i^{-}_1}$, ..., $\bbe_{i^{-}_{K}}$.
$B$ items are randomly sampled from the user's browsed items $i_{u,1}$,...,$i_{u,B}$.
These browsed items are encoded and gathered to $\bbE_u = [\bbe_{i_{u,1}},...,\bbe_{i_{u,B}}] \in \bbR^{B \times h}$.
\subsubsection{User Encoder}
The user encoder leverages users' interacted items to produce a content-aware user representation.
The final user representation is a weighted sum of the $B$ browsed items:
$$
\bbe_u = \sum_{b=1}^{B} \alpha_{b} \bbe_{i_{u,b}},
$$
where $\alpha_b$ is the attention weight assigned to $i_{u,b}$ that is obtained by passing features through two linear layers:
$$
\alpha_b = \frac{\exp{(\hat{\bbA}_b)}}{\sum_{b'=1,..,B}\exp{(\hat{\bbA}_{b'})}};
$$
$$
\hat{\bbA} = \tanh(\bbE_u \bbA_{fc_1}+\bbb_{fc_1})\bbA_{fc_2}+\bbb_{fc_2} \in \bbR^{B \times 1},
$$
where $\bbA_{fc_1} \in \bbR^{h\times \frac{1}{2}h}$, $\bbb_{fc_1} \in \bbR^{\frac{1}{2}h}$, $\bbA_{fc_2} \in \bbR^{\frac{1}{2}h\times 1}$, and $\bbb_{fc_2} \in \bbR^{1}$ are weights and biases of two fully-connected layers, respectively.

\subsubsection{Model Optimization}
% Having modelled the representations of users from their interacted items, 
The rating is the dot product of user and item embeddings:
$
\hat{y}_{ui} = (\bbe_u)^\mathsf{T} \cdot \bbe_i.
$
Assume that the scores of the positive samples and negative samples are $\hat{y}^{+}$ and $\hat{y}^{-}_{1}$,...,$\hat{y}^{-}_{K}$, following \cite{wu-etal-2019-neural-news}, the loss for optimization is the log posterior click probability of item $i$:
$$
\ccalL_{NRMS} = -\sum_{i \in \ccalS_i} \log{(\frac{\exp{(\hat{y}^{+})}}{\hat{y}^{+}+\sum_{k=1,..,K}\exp{(\hat{y}^{-}_{k})}})}
$$

\subsection{Fusion of CF and CBF: Content-Aware KMPN}
\label{sec:merge_model}
To fuse the information from a CBF model (NRMS-BERT) to a CF model (KMPN), the difficulty arises from the inconsistency of two models.
Co-optimizing two models by merging their output embeddings is an appealing idea, but however, this is not promising:

(1) KMPN requires much more epochs to converge than NRMS-BERT, though the cost per epoch of KMPN is significantly less.
This inconsistency in convergence leans the model's expressiveness to NRMS-BERT, leading to a decreased performance compared to KMPN alone in our preliminary experiments.

(2) CBF models that utilize large transformers can not be co-optimized with KG-based CF models, as graph convolution requires all embeddings to be present before convolution and this requires enormous GPU memory for even one single forward pass.

(3) Fusing pre-trained features from two models did not perform any better since the user/item representations has been determined in prior supervised training. Applying traditional aggregation methods (e.g., concatenation, MLP layers, multi-head attention) to combine features from two distinct systems broke the already-learned expressiveness and therefore showed worse performance in our preliminary experiments.

Therefore, a better way to fuse features is required, in line with three principles to make training efficient: (1) not optimizing two models together; (2) fusing features without learning towards the expressiveness of NRMS-BERT (3) not applying traditional feature aggregation on pre-trained embeddings.

Here, in line with our expectation to use a CF model for movie/book recommendation, we present a novel and efficient approach of fusing information for training a better KMPN: \textit{Cross-System Contrastive Learning}.
KMPN is still used as the framework backbone, and it is trained with the aid of a pre-trained NRMS-BERT.

In KMPN training,
for user and item in $(u, i^{+}, i^{-})\in \ccalU$,
embeddings are generated from NRMS-BERT: $e_u^{NRMS}$, $e_{i^{+}}^{NRMS}$, $e_{i^{-}}^{NRMS}$, and from KMPN: $e_u^{KMPN}$, $e_{i^{+}}^{KMPN}$, and $e_{i^{-}}^{KMPN}$.

\textit{Cross-System Contrastive Loss} is adopted to encourage KMPN system learns to incorporate content-aware features from NRMS-BERT features:
\begin{equation}
\begin{aligned}
    \ccalL_{CS}=\sum_{(u, i^{+}, i^{-})\in \ccalU} &-\ln \Big (\sigma \big ((\bbe_u^{KMPN})^\mathsf{T} \cdot \bbe_{i^{+}}^{NRMS}-(\bbe_u^{KMPN})^\mathsf{T} \cdot \bbe_{i^{-}}^{NRMS}\big) \Big) \\
    &-\ln \Big (\sigma \big ((\bbe_u^{NRMS})^\mathsf{T} \cdot \bbe_{i^{+}}^{KMPN}-(\bbe_u^{NRMS})^\mathsf{T} \cdot \bbe_{i^{-}}^{KMPN}\big) \Big)
\end{aligned}
\label{eqn:cross_system_loss}
\end{equation}

This loss encourages KMPN to produce item embeddings that can not only interact with its own user embeddings, but also with NRMS-BERT's user embeddings.
Similarly, user embeddings of KMPN are trained to interact with items of NRMS-BERT.
It allows $\bbe_i^{KMPN}$ to learn mutual expressiveness with $\bbe_i^{NRMS}$, but without approaching the two embeddings directly using similarity (e.g. cosine-similarity), which has been proved to damage the performance in experiments.
In this case, $\bbe_u^{NRMS}$ serves as a bridge with which the item embeddings of two systems learn to share commons and increase their mutuality.

A more mathematical explanation states that this loss encourages $\bbe_i^{KMPN}$ and $\bbe_i^{NRMS}$ to lie in the same hidden space hyperplane on which features have the same dot-product results with $\bbe_u^{NRMS}$.
This contrastive constraint optimizes KMPN to grow embeddings in the same region of hidden space, leading to mutual experessiveness across two systems.


Finally, the optimization target is:
$$
\ccalL_{CKMPN} = \ccalL_{KMPN} + \lambda_{CS}\ccalL_{CS},
$$
where $\lambda_{CS}$ controls the weight of the Cross-System Contrastive Loss.



% Context-Aware Knowledge-Graph-Enhanced Meta-Preference Network


\section{Experiments}

\begin{table*}[!ht]
\caption{Comparison of baseline models and our proposed models on Amazon-Book-Extended dataset. Numbers \underline{underlined} are existing state-of-the-art performance, while best performance of the proposed models are marked in \textbf{bold}.
Relative improvements over models are shown in the last two rows.
}
\label{tab:compare_baselines}
\small
\centering
\begin{tabular}{llllllllll}
\toprule
                                  & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{ndcg}   & \multicolumn{3}{c}{Hit Ratio}  \\
~                                 & @20   & @60   & @100    & @20   & @60     & @100  & @20   & @60   & @100        \\
\midrule
BPRMF                                & 0.1352&	0.2433&	0.3088&	0.0696&	0.09568&	0.1089&	0.2376&	0.3984&	0.4816

          \\
CKE                               & 0.1347&	0.2413&	0.3070&	0.0691&	0.09482&	0.1081&	0.2373&	0.3963&	0.4800
            \\
KGAT                              & 0.1527&	0.2595&	0.3227&	0.0807&	0.10655&	0.1194&	0.2602&	0.4156&	0.4931
       \\
KGIN                              & \underline{0.1654}&	\underline{0.2691} &	\underline{0.3298} &	\underline{0.0893} &	\underline{0.1145} &	\underline{0.1267} &	\underline{0.2805} &	\underline{0.4289} &	\underline{0.5040}
       \\
\midrule
KMPN & \textbf{0.1719} & 0.2793 & 0.3405   & \textbf{0.0931} & 0.1189 & 0.1315 & \textbf{0.2910} & 0.4421 & 0.5166       \\
- SoftDistanceCorrelation  & 0.1704 & 0.2790 & 0.3396   & 0.0924 & 0.1185  & 0.1310 & 0.2881 & 0.4419 & 0.5152       \\
- ReciprocalRatioNegativeSampling                              & 0.1690 & 0.2774 & 0.3391   & 0.0913 & 0.1177  & 0.1302 & 0.2872 & 0.4414 & 0.5155       \\
% KMPN                              & 0.1690 & 0.2774 & 0.3391   & 0.0913 & 0.1177  & 0.1302 & 0.2872 & 0.4414 & 0.5155       \\
% +ReciprocalRatioNegativeSampling  & 0.1704 & 0.2790 & 0.3396   & 0.0924 & 0.1185  & 0.1310 & 0.2881 & 0.4419 & 0.5152       \\
% +SoftDistanceCorrelation          & \textbf{0.1719} & 0.2793 & 0.3405   & \textbf{0.0931} & 0.1189 & 0.1315 & \textbf{0.2910} & 0.4421 & 0.5166       \\
\midrule
NRMS-BERT &	0.1142 &	0.2083	& 0.2671 &	0.0592 &	0.0817 &	0.0935 &	0.2057 &	0.3487 &	0.4273 \\
\midrule
CKMPN ($\lambda_{CS}=0.2$) & 0.1699 & 0.2812 & \textbf{0.3461}   & 0.0922 & 0.1190 & 0.1319 & 0.2880 & 0.4460 & 0.5235       \\
CKMPN ($\lambda_{CS}=0.1$) & 0.1718 & \textbf{0.2821} & 0.3460   & 0.0928 & \textbf{0.1197} & \textbf{0.1326} & 0.2908 & \textbf{0.4474} & \textbf{0.5244}   \\
\midrule
Improv. (\%) CKMPN v.s. Baselines &	3.90&	4.82&	4.94&	4.31&	4.55&	4.59&	3.72&	4.33&	4.04
\\
Improv. (\%) CKMPN v.s. KMPN & 0.0	& 1.0 &	1.6	 & -0.3	 & 0.7 &	0.8 &	0.0	& 1.2 &	1.5\\
\bottomrule
\end{tabular}
\end{table*}
In this section, we present experimental results of the three proposed models: KMPN, NRMS-BERT, and CKMPN, with detailed discussions.
We firstly demonstrate model improvements over existing baseline models including state-of-the-art models on Amazon-Book-Extended, which has an extensive record of publications that enables direct and fair comparison.
Then we provide benchmark results on our brand-new Movie-KG-Dataset to enable the development and comparison of future models.


\subsection{Evaluation Metrics}
Following common practice~\cite{he2017neural, wang2019kgat, wang2021learning}, we report several metrics (algorithms summarized in \cite{krichene2020sampled}) for evaluating model performance:

\textit{Recall@K}: within top-$K$ recommendations, how well the system is able to recall the test-set browsed items for each user.

\textit{ndcg@K} (Normalized Discounted Cumulative Gain): increases when relevant items appear more earlier in the recommended list. 

% \textit{Precision@K}: how relevant the recommended top-$K$ items are to the specific user.

\textit{HitRatio@K}: how probable the user click through one of the recommended top-$K$ items.

\subsection{Baselines}
We take the performance of several recently published recommender systems as points for comparison.
We carefully reproduced all these baseline systems from their official repository.\footnote{As a result, the metrics reported in this paper may differ from what were presented in the original papers.}

\textbf{BPRMF}~\cite{rendle2012bpr}: an advanced matrix factorization method that applies a generic optimization criterion BPR-Opt for personalized ranking that derives from Bayesian analysis.


\textbf{CKE}~\cite{zhang2016collaborative}: a CF model that aims to leverage heterogeneous information in a knowledge base for recommendation.

\textbf{KGAT}~\cite{wang2019kgat}: Knowledge Graph Attention Network (KGAT) which explicitly models the high-order connectivities in KG in an end-to-end fashion. The models' user/item embeddings were initialized from the pre-trained \textbf{BPRMF} weights.

\textbf{KGIN}~\cite{wang2021learning}: A state-of-the-art CF model that models users' latent intents as a combination of KG relations.



% \subsection{Training Details}
% All experiments were run on 8 NVIDIA A100 Tensor Core GPUs with batch size $8192\times 8$ for KMPN/CKMPN and $4\times8$ for NRMS-BERT.
% KMPN/CKMPN's optimizer was Adam \cite{DBLP:journals/corr/KingmaB14} with 2000 epochs of linearly decayed learning rate from $10^{-3}$ to $0$ for Amazon-Book-Extended and $5\times10^{-4}$ to $0$ for Movie-KG-Dataset.
% NRMS-BERT was optimized with Adam at a constant learning rate of $10^{-4}$.
% Codes will be released with all training details upon publication.


\subsection{Model Performance on Amazon Dataset}

\begin{table*}[!ht]
\caption{Benchmark results on Movie-KG-Dataset. Best performance is marked in \textbf{bold}.
}
\label{tab:compare_baselines_movies}
\centering
\small
\begin{tabular}{llllllllll}
\toprule
                                  & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{ndcg}   & \multicolumn{3}{c}{Hit Ratio}  \\
~                                 & @20   & @60   & @100    & @20   & @60     & @100  & @20   & @60   & @100        \\
\midrule
BPRMF                                & 0.1387 &	0.1944&	0.2206&	0.0961&	0.1137&	0.1192&	0.1980&	0.2785&	0.3236
          \\
CKE & 0.1369&	0.1898&	0.2150&	0.0940&	0.1108&	0.1160&	0.1950&	0.2707&	0.3155
\\
KGAT&	\underline{0.1403}&	0.1928&	0.2185&	\underline{0.1006}&	0.1173&	0.1226&	0.1997&	0.2742&	0.3196
\\
KGIN&	0.1351&	\underline{0.2119}&	\underline{0.2445}&	0.0982&	\underline{0.1254}&	\underline{0.1322}&	\underline{0.2194}&	\underline{0.3081}&	\underline{0.3643}\\

\midrule
KMPN & 0.1434&	0.2130&	0.2427&	0.1073&	0.1305&	0.1367&	0.2193&	0.3098&	0.3602
\\
NRMS-BERT& 0.0941&	0.1456&	0.1598&	0.0754&	0.0914&	0.0945&	0.1541 & 0.2034&	0.2348
\\
CKMPN & \textbf{0.1463}&	\textbf{0.2153}&	\textbf{0.2467}&	\textbf{0.1087}&	\textbf{0.1334}&	\textbf{0.1402}&	\textbf{0.2211}&	\textbf{0.3124}&	\textbf{0.3657}
\\



\bottomrule
\end{tabular}

\end{table*}





Performance of models is presented in Table~\ref{tab:compare_baselines}. 
Our proposed CF model, KMPN, with \textit{Reciprocal Ratio Negative Sampling} and \textit{Soft Distance Contrastive Learning}, achieved a significant improvement on all metrics over the performance of the existing state-of-the-art model KGIN, for example, Recall@20 was improved from 0.1654 to 0.1719, Recall@100 from 0.3298 to 0.3405, and ndcg@100 from 0.1267 to 0.1315.

% As shown, enhanced by knowledge graph, our proposed collaborative-filtering model KMPN achieved an improvement on all metrics over the performance of the existing state-of-the-art model KGIN, for example, Recall@100 was improved from 0.3298 to 0.3391 and Hit Ratio@100 from 0.5040 to 0.5155.

NRMS-BERT models user-item preferences through only summary texts of items, without external information from a knowledge base.
It still achieves 0.1142 in Recall@20 and 0.4273 Hit Ratio@100, not far from the KGIN baseline at 0.5040 Hit Ratio@100. 
It suggests that our extension to Amazon-Book dataset serves as a good additional content-based source for constructing recommendation systems.

Finally, our proposed \textit{Cross-System Contrastive Learning} approach significantly improves all @60/@100 metrics while keeping model's performance of @20.
For example, as shown, CKMPN achieved 0.1718 in Recall@20, the same as the best configuration of KMPN.
But CKMPN (0.3461 Recall@100) outperforms KMPN (0.3405 Recall@100) by 1.6\%.
This demonstrates that by gathering item and user embeddings of one system (KMPN) towards those of the other system (NRMS-BERT) through proxies (Cross-System Contrastive Learning) encourages KMPN to learn and fuse content-aware features from the learnt representations of a CBF model.
The fuse of this content-based feature significantly enhanced KMPN's ability to gather more relevant items into the top-$100$ recommendation list.
This improvement on top-$60/100$ metrics is appealing to the industry where a relatively large amount of items are firstly recalled by a Recall Model and then a Ranking Model is adopted to refine the list ranking.

In the following subsections, we briefly explore the effects brought by the hyperparameters in order to support the rationale of our designs for KMPN.




\subsubsection{Effects of Reciprocal Ratio Negative Sampling}
\label{sec:experiments:negative_sampling}
Through \textit{Reciprocal Ratio Negative Sampling}, KMPN further improves the metrics: Recall@20 increases from 0.1690 to 0.1704.
In line with our intuition, reducing the probability of sampling popular items as negative samples for training can significantly benefit the model learning.
This demonstrates that while viewed-but-not-clicked samples are not available to the model, \textit{Reciprocal Ratio Negative Sampling} is a good protocol that enhances the quality of negative samples.
% produced by commonly-used sampling strategies.

\subsubsection{Effects of Meta Preferences}
\label{sec:experiments:meta_preferences}



\begin{figure}
\centering     %%% not \center

\subfigure[Model performance varies with the number of meta-preferences. Best performance is obtained at $N_m=64$.]{\label{fig:effects_of_meta_preference}\includegraphics[width=0.48\linewidth]{content/figures/meta_preferences_compare.png}}
\hfill
\subfigure[Model performance varies with the ratio $\epsilon$ of Soft Distance Correlation.
$\epsilon=0$ trains preference embeddings without Distance Correlation Loss; $\epsilon=1$ reduces to Distance Correlation.
]{\label{fig:effects_of_soft_distance_correlation}\includegraphics[width=0.48\linewidth]{content/figures/PCA_compare.png}}
\vspace{-0.5cm}
\caption{Hyperparameter evaluation with number of meta-preferences and Soft Distance Correlation.}
\label{fig:effects_hyperparameters}
\vspace{-0.5cm}
\end{figure}

% \begin{figure*}
% \centering     %%% not \center
% \begin{minipage}{0.61\textwidth}
% \caption{Benchmark results on Movie-KG-Dataset. Best performance is marked in \textbf{bold}.}
% \label{tab:compare_baselines_movies}
% \centering
% % \small
% \footnotesize
% \begin{tabular}{llllllllll}
% \toprule
%                                   & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{ndcg}   & \multicolumn{3}{c}{Hit Ratio}  \\
% ~                                 & @20   & @60   & @100    & @20   & @60     & @100  & @20   & @60   & @100        \\
% \midrule
% BPRMF                                & 0.1387 &	0.1944&	0.2206&	0.0961&	0.1137&	0.1192&	0.1980&	0.2785&	0.3236
%           \\
% CKE & 0.1369&	0.1898&	0.2150&	0.0940&	0.1108&	0.1160&	0.1950&	0.2707&	0.3155
% \\
% KGAT&	\underline{0.1403}&	0.1928&	0.2185&	\underline{0.1006}&	0.1173&	0.1226&	0.1997&	0.2742&	0.3196
% \\
% KGIN&	0.1351&	\underline{0.2119}&	\underline{0.2445}&	0.0982&	\underline{0.1254}&	\underline{0.1322}&	\underline{0.2194}&	\underline{0.3081}&	\underline{0.3643}\\

% \midrule
% KMPN & 0.1434&	0.2130&	0.2427&	0.1073&	0.1305&	0.1367&	0.2193&	0.3098&	0.3602
% \\
% NRMS-BERT& 0.0941&	0.1456&	0.1598&	0.0754&	0.0914&	0.0945&	0.1541 & 0.2034&	0.2348
% \\
% CKMPN & \textbf{0.1463}&	\textbf{0.2153}&	\textbf{0.2467}&	\textbf{0.1087}&	\textbf{0.1334}&	\textbf{0.1402}&	\textbf{0.2211}&	\textbf{0.3124}&	\textbf{0.3657}
% \\



% \bottomrule
% \end{tabular}
% \end{minipage}
% \hfill
% \begin{minipage}{0.37\textwidth}
% \subfigure[]{\label{fig:effects_of_meta_preference}\includegraphics[width=0.49\linewidth]{content/figures/meta_preferences_compare.png}}
% \subfigure[]{\label{fig:effects_of_soft_distance_correlation}\includegraphics[width=0.49\linewidth]{content/figures/PCA_compare.png}}
% \caption{Hyperparameter evaluation with number of meta-preferences and Soft Distance Correlation.}
% \label{fig:effects_hyperparameters}
% \end{minipage}
% \end{figure*}

An obvious research question is how the design of modelling user through meta-preferences improves the model performance.

As shown in Fig.~\ref{fig:effects_of_meta_preference}, $N_m=16$ achieved worse performance than $N_m\geq32$ due to the limited capacity of modelling user preference.
Peaking at $N_m=64$, the performance started to decrease at $N_m\geq128$, which suggests that bringing too many preference bridges induces overfitting and will not further improve the system, and a moderate $N_m$ is suificient for best performance.


% $\epsilon=0$ is the model where all preference embeddings $\{\bbe_{p}\in \bbR^{h}|p\in \ccalP \}$ are directly trainable instead of a distribution over meta-preferences.


\subsubsection{Effects of Soft Distance Correlation Loss}
\label{sec:experiments:soft_distance_correlation}
The hyperparameter $\epsilon$ controls the number of primary components to keep after PCA dimension reduction.
The lower the ratio, the more flexibility the preference embeddings will recover in dimensions from the standard Distance Correlation constraint.
$\epsilon=0$ removes the Soft Distance Correlation Constraint on preference embeddings completely, while $\epsilon=1$ reduces to a standard Distance Correlation Loss. 
As shown in Fig.~\ref{fig:effects_of_soft_distance_correlation},
the model performance peaks at $\epsilon = 0.5$, where half of $h$ dimensions are relaxed from the Distance Correlation constraint, and preference embeddings are still able to grow diversely in the remaining half dimensions.
As $\epsilon$ approaches 0, the Distance Correlation constraint becomes too loose to encourage the diversity of preferences, leading to a dramatically decreased performance.

\subsubsection{Effects of Cross-System Contrastive Learning}
\label{sec:experiments:cross_system_learning}
\begin{figure}
\centering     %%% not \center
\subfigure[Recall@20 (blue) and ndcg @20 (red)
]{\label{fig:effects_of_cs_loss_20}\includegraphics[width=0.48\linewidth]{content/figures/cs_loss_@20.png}}
\hfill
\subfigure[Recall@100 (blue) and ndcg @100 (red)]{\label{fig:effects_of_cs_loss_100}\includegraphics[width=0.48\linewidth]{content/figures/cs_loss_@100.png}}
\vspace{-0.5cm}
\caption{System performance against the loss weight $\lambda_{CS}$ of Cross-System Contrastive Loss. The performance at top-$100$ (right) is greatly improved while keeping the metrics of top-$20$ (left) steady until $\lambda_{CS}>0.2$.}
\label{fig:effects_of_cs_loss}
\vspace{-0.3cm}
\end{figure}

We experimented with different $\lambda_{CS}$ in order to find the best configuration for the Cross-System Contrastive Loss.
As shown in Fig.~\ref{fig:effects_of_cs_loss_20}, the system performance of top-$20$ did not drop much until $\lambda_{CS}>0.2$. But meanwhile, Fig.~\ref{fig:effects_of_cs_loss_100} demonstrates that the performance at top-$100$ increases dramatically at $\lambda_{CS}\leq 0.2$ compared to the system without the Cross-System Contrastive Loss.

Therefore, we can easily conclude that by contrastively learning cross-system user/item representations around proxies that provide anchors, CKMPN successfully fuses the external information from a content-based system, NRMS-BERT, and the improvement on all @60/@100 metrics over KMPN arises from the mutual context-aware features learned from both systems.
It is also worth noting that this contrastive learning loss is not only limited to fusing textual modality, but can be applied to any other modalities that provide already good item/user representations for recommendation.
% after proper supervised training.


% \begin{table*}[!ht]
% \caption{Benchmark results on Movie-KG-Dataset. Best performance is marked in \textbf{bold}.
% }
% \label{tab:compare_baselines_movies}
% \centering
% \begin{tabular}{llllllllll}
% \toprule
%                                   & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{ndcg}   & \multicolumn{3}{c}{Hit Ratio}  \\
% ~                                 & @20   & @60   & @100    & @20   & @60     & @100  & @20   & @60   & @100        \\
% \midrule
% BPRMF                                & 0.1699&	0.2063&	0.2251&	0.1458&	0.1577&	0.1616&	0.2169&	0.2724&	0.3082

%           \\
% CKE & 0.1708&	0.2114&	0.2333&	0.1407&	0.1536&	0.1582&	0.2195&	0.2832&	0.3240\\
% KGAT&	0.1857&	0.2347&	0.2630&	0.1562&	0.1708&	0.1767&	0.2465&	0.3244&	0.3739\\
% KGIN&	0.1968&	0.2525&	0.2818&	0.1595&	0.1762&	0.1823&	0.2680&	0.3522&	0.4022\\
% \midrule
% KMPN & \textbf{0.2006}&	0.2539&	0.2827&	0.1618&	\textbf{0.1781}&	0.1841&	0.2696&	0.3538&	0.4033\\
% NRMS-BERT&0.1482&	0.1880&	0.2068&	0.1227&	0.1369&	0.1407&	0.2066&	0.2603&	0.2953
% \\
% CKMPN & 0.1999 &	\textbf{0.2545}&	\textbf{0.2836}&	\textbf{0.1619}&	0.1779&	\textbf{0.1842}&	\textbf{0.2699}&	\textbf{0.3555}&	\textbf{0.4050}\\



% \bottomrule
% \end{tabular}

% \end{table*}

\subsection{Benchmarking on Movie-KG-Dataset}

After verifying the effectiveness of our proposed models in Amazon-Book-Extended, we report their best performance on the newly collected movie dataset (Standard version with 19 days).\footnote{Extended version (39 days) will be released upon publication for larger applications.}
The performance of the same baseline systems is provided for inclusion (Table ~\ref{tab:compare_baselines_movies}).
The same performance boost is observed on KMPN over baselines.
CKMPN also achieved the best performance with the content-based features from NRMS-BERT.
We can conclude that our method is generalizable in different datasets.

\section{Conclusion}
In order to explore fusing CBF into CF models for movie/book recommendation, this paper presented two datasets: (1) Amazon-Book-Extended which inherited from a popular book recommendation dataset and was newly extended by summary texts of books; (2) a brand-new large-scale movie recommendation dataset, Movie-KG-Dataset, which was recently collected from user browser history and provides an enormous knowledge graph together with summary texts for movies.
Both datasets will be shared with the research community in order to facilitate the domain research.

To utilize the power of large transformer models in context-aware collaborative filtering,
this paper firstly proposed and evaluated a powerful CF model, KMPN, which utilizes \textit{Gated Path Graph Convolution Networks}, \textit{Soft Distance Correlation Loss}, and \textit{Reciprocal Ratio Negative Sampling} to outperform existing baseline models.
Then, a novel approach, \textit{Corss-System Contrastive Learning} of embeddings was proposed to fuse content-aware features from a CBF model, NRMS-BERT, and achieved the best performance in record.
We finally presented benchmark results on both datasets for comparison with future research.
